Higgs boson potential at colliders: status and perspectives

This document summarises the current theoretical and experimental status of the di-Higgs boson production searches, and of the direct and indirect constraints on the Higgs boson self-coupling, with the wish to serve as a useful guide for the next years. The document discusses the theoretical status, including state-of-the-art predictions for di-Higgs cross sections, developments on the effective field theory approach, and studies on specific new physics scenarios that can show up in the di-Higgs final state. The status of di-Higgs searches and the direct and indirect constraints on the Higgs self-coupling at the LHC are presented, with an overview of the relevant experimental techniques, and covering all the variety of relevant signatures. Finally, the capabilities of future colliders in determining the Higgs self-coupling are addressed, comparing the projected precision that can be obtained in such facilities. The work has started as the proceedings of the Di-Higgs workshop at Colliders, held at Fermilab from the 4th to the 9th of September 2018, but it went beyond the topics discussed at that workshop and included further developments.

==> AnalysisTechniques/sigma_kl.tex <==
\subsection[Signal simulation and cross section parameterisation as a function of $\klambda$]{Signal simulation and cross section parameterisation as a function of $\klambda$ \\ \contrib{B. Di Micco}}
In the gluon-gluon fusion $HH$ production, the production process depends on two amplitudes as described in Sec.~\ref{sec:non_res:comb}.
In case of a varied trilinear coupling $\lambda_{HHH}$ modified by a coefficient $\klambda = \lambda_{HHH}/\lambda_{HHH}^\rm{SM}$ this allows to express the differential and inclusive  $pp \to HH$ cross section as a second degree  polynomial in $\klambda$.
\[
\frac{d\sigma}{d\Phi} = A + B\klambda + C \klambda^2
\]
where $d\Phi$ represents the infinitesimal phase space volume. This expression is valid at all order in QCD, higher order QCD corrections will affect, in fact,  the values of the $A,B,C$ coefficients but not the functional dependence from $\klambda$. This feature can be used to simulate MC samples for any values of $\klambda$ using three samples generated for three different values of $\klambda$ by solving the following system of equations:

\begin{eqnarray}
\left (\frac{d\sigma}{d\Phi}\right )_1 = A + B\kappa_{\lambda 1} + C \kappa_{\lambda 1}^2 \\
\left (\frac{d\sigma}{d\Phi}\right )_2 = A + B\kappa_{\lambda 2} + C \kappa_{\lambda 2}^2 \\
\left (\frac{d\sigma}{d\Phi} \right)_3 = A + B\kappa_{\lambda 3} + C \kappa_{\lambda 3}^2 \\
\end{eqnarray}
and computing the dependence of the coefficient $A,B,C$ from the differential cross section in a given phase space volume. In practice this is achieved by linearly combining the three reference samples with coefficients obtained by the inversion of the matrix above. A natural choice for two $\klambda$ values of the reference samples is $\klambda = 0, 1$, corresponding to the box-only and the SM cases. In order to optimise the signal generation, the third value can be chosen close to the expected exclusion region. For the current LHC sensitivity this corresponds to $\klambda = 10, 20$ according to the channel sensitivity.

The three samples need to be properly normalised to the best cross section computations, these can be also paramaterised as a second degree polynomial with coefficients $a,b,c$. 
Figure~\ref{fig:cross_plots} shows the comparison of several cross section curves.
The LO computation, the NNLO+NNLL computation in the $m_t \to \infty$ approximation rescaled with the NNLO+NNLL SM cross section obtained including finite $m_t$ NLO contribution and $m_t \to \infty$ NNLO corrections,  and the last computation obtained with the finite $m_t$ NLO computation for all $\klambda$ values rescaled with the NNLO SM cross section obtained with the FTApprox method (partial $m_t$ finite). 

The corresponding second degree polynomial parameters are shown in Tab.~\ref{tab:cross_parab_summary}

\begin{figure}[hbt]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/cross_comp.pdf}
     \includegraphics[width=0.45\textwidth]{figures/ratio_comp.pdf}
    \caption{Left: $pp \to \hh$ production cross section as a function of $\klambda$. Right: ratio of the  $pp \to \hh$  to its SM expectation, obtained for $\klambda =1$. Different calculations, as used by the LHC experiments are shown. }
    \label{fig:cross_plots}
\end{figure}

\begin{table}[hbt]
    \centering
    \begin{tabular}{lccc}
    \hline
    computation & a [fb] & b [fb] & c [fb] \\
    \hline
    LO $m_t$ fin  & 34.9836 & -22.9863 & 4.72815 \\
    NLO $m_t$ fin & 62.6094 & -44.3898 & 9.64419 \\
    NLO $m_t$ fin $\times$ NNLO SM FTApprox & 69.9791 & -49.6149 & 10.7794 \\
    NNLO + NNLL $m_t \to \infty$ $\times$ NNLO+NLL SM (partial $m_t$ fin) & 71.3591 & -47.7427 & 9.9315 \\
    \hline
    \end{tabular}
    \caption{Second order polynomial parameters ($a+b\cdot \klambda + c\cdot \klambda^2$) for different computations as used by the experimental collaborations and new recommendations.}
    \label{tab:cross_parab_summary}
\end{table}
\clearpage

==> HHFuture/HHinee-MEP.tex <==

\label{chap:ee}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}


\section{Introduction}

The  Higgs self-coupling can be measured at $e^+e^-$  colliders in two
different ways. First, the coupling can be measured directly, using 
processes with Higgs pair production
that  include diagrams involving  the Higgs self-coupling at the tree level. 
Second, the coupling can be measured indirectly, using 1-loop 
radiative corrections to single Higgs processes that include the Higgs
self-coupling as a vertex.    

The direct measurement requires
high centre-of-mass energies,  500~GeV or above, that
should be provided by the proposed linear $e^+e^-$ colliders 
 ILC and CLIC.    The indirect
determination applies to any facility that can make sufficiently
precise measurements of the rates of single-Higgs processes.  Thus, it 
applies to the proposed circular colliders CEPC and FCC-ee as well as
to the linear colliders. 

In addition to quantitative improvements, the measurement of the Higgs
self-coupling at $e^+e^-$ colliders offers two unique advantages with
respect to the measurements at hadron colliders.   The first of these
comes 
in direct Higgs pair production. 
There are two  important Higgs pair production reactions at $e^+e^-$ colliders,
$e^+e^-\to ZHH$ and $e^+e^-\to \nu\bar\nu HH$. 
For both reactions, diagrams that
do not involve the Higgs self-coupling appear in interference with diagrams that do
contain this coupling.   An interesting feature is that, in the $ZHH$ process the
interference is constructive, while in the $\nu\bar\nu HH$ the interference is
destructive.  Then, no matter what is the sign of the deviation of the Higgs self-coupling from its SM value, one process is always enhanced and offers a good
setting to measure the effect.   

The second unique advantage appears when either the direct or the
indirect method is applied in a complete program of measurements of
the properties of the Higgs boson. 
As has been stressed already in this report, it is not possible to
extract the value of the Higgs self-coupling from a measurement of an
\hh production cross section unambiguously  without considering other possible
beyond-SM effects on that cross section.  Ideally, one should perform
 a general analysis in the context of Effective Field Theory.   As we
 have reviewed in Sec.~\ref{sec:smeft}, the value of the Higgs self-coupling is
 controlled in the SMEFT by a parameter $c_6$.  Recalling Eq.~\leqn{eq:klrel},
 \beq
 \kappa_\lambda = 1 +  c_6  - \frac{3}{2} c_H + \cdots \ . 
 \eeq{recallklrel}
The parameter  $c_6$ originates from an operator that modifies the Higgs
 potential,  $c_H$ is a universal rescaling of all Higgs
 couplings that originates from a modification of the Higgs field
 kinetic term, and the omitted terms represent additional electroweak
 corrections not included in the simplified framework of Sec.~\ref{sec:smeft}.
 We saw in that section that the SMEFT contains many other 
parameters that influence the value of the \hh
production cross section.  Ideally, one should account for the
dependence of the \hh cross section on all of these parameters, 
constraining parameters other than $c_6$.    This is even more
 important for the extraction of $c_6$  from radiative
 corrections to single Higgs production processes, since many SMEFT
 parameters can affect these processes at the tree level while the effect of
 $c_6$ comes only at the 1-loop level.

Because of the high precision expected at an $e^+e^-$ collider
for the measurements of the
other Higgs boson couplings, across the full range of these couplings, 
this global fit for the Higgs self-coupling can be made very tight.
Indeed,  it is
likely that information from $e^+e^-$ measurements will also be needed to
interpret the hadronic measurements of \hh production discussed
earlier in this report. 

In this section we will discuss all of these aspects in turn.   We
will first discuss the direct measurement of the Higgs self-coupling
through \hh pair production, reviewing the studies that have been
done for the proposed linear $e^+e^-$ colliders ILC and CLIC.  We will
present
the results obtained in the context of an EFT with only the value of the
self-coupling varying from its SM value.   We will then discuss the
interpretation of these measurements within a global SMEFT fit that
includes input from the $e^+e^-$ measurements of single Higgs production
and other electroweak processes.   Next, we will discuss global fits
to single Higgs observables and the possibility of obtaining model-independent
constraints on $c_6$ from these fits.  Finally, we will put the
whole picture together and give combined projections for the accuracy
with which $c_6$ can be determined at proposed linear and
circular $e^+e^-$ colliders.

\section{$HH$ production processes at $e^+e^-$ colliders}
\label{sec:genHHee}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.62\hsize]{HHFuture/fig/CrossSectionPlot.pdf}
\vspace*{-0.3cm}
\caption{Cross sections for the double Higgs production processes
  $e^+e^- \to ZHH$ and $e^+e^- \to \nu\bar{\nu}HH$, as a function of
  $\sqrt{s}$ for $m_H=125\,$GeV.   The cross sections are shown for
unpolarized beams.  These cross sections are higher -- in the latter
case, by almost a factor 2 -- when the $e^-$ beam is highly polarized
in the left-handed sense. } 
\label{fig:sigzhh_vvhh}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The cross sections for the $ZHH$ and $\nu\bar\nu HH$ production
processes at $e^+e^-$ colliders 
are shown in Fig.~\ref{fig:sigzhh_vvhh}.   The cross sections are
shown in this figure for unpolarized beams.   Planned analyses at
$e^+e^-$ colliders will make use of polarized beams.  Since the
$\nu\bar\nu HH$ process, in particular, requires the initial state
$e^-_Le^+_R$, working with polarized beams can raise the cross section
significantly, by almost a factor of 2.  Still, these cross sections
are very small, and the processes are difficult to recognize even in
the relatively clean environment of an $e^+e^-$ collider.


 The $ZHH$ process  can be studied already at an $e^+e^-$ centre of mass energy of
500~GeV.   The $\nu\bar\nu HH$ reaction, which 
is a 4-body process, requires  higher energy.   The ILD group has
studied these reactions at $\sqrt{s}$ energies of
500~GeV and 1~TeV~\cite{Tian:2013qmi, KurataHHH,Duerig:2016dvi}.    The
CLICdp group has studied these reactions at $\sqrt{s}$ energies of 1.5~TeV and
3.0~TeV~\cite{Roloff:2019crr}.   We will describe these analyses
below.
In both cases, the
analyses are done in the framework of full simulation using detailed
detector models.   This simulation framework is reviewed in Secs.~6 and
7 of Ref.~\cite{Bambade:2019fyw}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.95\hsize]{HHFuture/fig/WWHH_feynman_diagrams.png}
\caption{Diagrams contributing to $e^+e^- \to \nu\bar{\nu}hh$.} 
\label{fig:hhdiagrams}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The diagrams for both processes  include a diagram with
the Higgs self-coupling in interference with diagrams in which the two
Higgs bosons are radiated separately from $W$ or $Z$ propagators.  The
SM diagrams for $e^+e^-\to \nu\bar\nu HH$ are shown in Fig.~\ref{fig:hhdiagrams}.
Note that both processes appear at the tree level in the SM and, since
we are in the electroweak world, the tree level is a good
approximation to the full result.   As noted above, the Higgs
self-coupling diagram interferes constructively with the other SM
diagrams in the case of $ZHH$ and destructively in the case of
$\nu\bar\nu HH$.   The dependence of the cross section on the  variation of
the Higgs self-coupling is shown in Fig.~\ref{fig:HHHBSM}.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
  \centering
    \includegraphics[width=0.7\hsize]{HHFuture/fig/xsec_coupling_BSM.pdf} 
    \vspace*{-0.3cm}
    \caption{The dependence of the cross sections for \hh production as a
      function of the Higgs self-coupling $\lambda$ for
      $e^+e^-\to ZHH$ ~(red line) and for 
      $e^+e^-\to\nu\bar{\nu}HH$ ~(blue line).
      The values of  both $\lambda$ and $\sigma$ are scaled to their 
      SM values. Note that the exact results depend on the assumed beam
    polarizations, here taken in the ILC scheme.}
  \label{fig:HHHBSM}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{$HH$ production --- ILC}
\label{sec:eedirectILC}

The International Linear Collider (ILC)
is an $e^+e^-$ linear collider based on superconducting RF technology,
aimed
at precision studies of the Higgs boson, the top quark, and other
standard
and exotic electroweak processes in the energy range 250~GeV to
500~GeV.  The ILC is now planned in two stages, the first of which
would operate at 250~GeV and the second of which would operate at
350~GeV, 500~GeV, and possibly at higher energies.   The technical
design report for the
ILC was completed in 2013~\cite{Behnke:2013xla}.  This report includes the design of an
ILC stage at 1~TeV.  A recent review of the ILC
design and capabilities can be found in \cite{Bambade:2019fyw}. 

Full simulation studies show that discovery of the
double Higgs-strahlung process is possible within the planned program
of the ILC at its second stage:   4~ab$^{-1}$ of data at a $\sqrt{s}$ energy
of 500~GeV.  The run plan assumes polarization of 80\% for the
electron beam and 30\% for the positron beam, with the beam
polarizations
divided  among LR/RL/LL/RR  polarizations as
40\%/40\%/10\%/10\%.  Using the ILD detector model in full-simulation
analyses, the ILD group studied the extraction of the $ZHH$ process
from background in the di-Higgs decay channels  $hh\to
b\bar{b}b\bar{b}$~\cite{Tian:2013qmi,Duerig:2016dvi} and $hh\to
b\bar{b}W^+W^-$~\cite{KurataHHH}.  At this point  in the ILC program,
the
absolute
branching ratios of the Higgs boson into the $b\bar b$ and $WW^*$
channels will already be known with sub-percent
accuracy~\cite{Bambade:2019fyw}.  The measurements of $\sigma\cdot BR$
for the two channels can then be applied directly to the \hh
production cross section.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.4\hsize]{HHFuture/fig/HmassforZHHlept.png}
  \quad
 \includegraphics[width=0.4\hsize]{HHFuture/fig/HmassforZHHhadr.png}
 \caption{Reconstruction of the Higgs boson mass in the measurements
  of the $e^+e^-\to ZHH$ cross section described in
\cite{Duerig:2016dvi}: left: highest energy Higgs boson in events
with $Z\to \ell^+\ell^-$; right: highest energy Higgs boson in
 events with  $Z\to q\bar q$. }
  \label{fig:eehmasses}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The measurement of the $ZHH$ cross section in the $b\bar{b}b\bar{b}$
is described in detail in the Ph.D. thesis of
D\"urig~\cite{Duerig:2016dvi}.   She presents three  paralled analyses for
the channels of $Z$ decay to charged leptons, to neutrinos, and to
quarks (including $b\bar{b}$.  In each case, a kinematic fit is
carried out on the 4- or 6-jet system, and the output parameters from  this fit
are  supplied to multivariate classifiers. The reconstructed Higgs
masses in the cases of charged leptonic and hadronic $Z$ decays are
shown in Fig.~\ref{fig:eehmasses}.   The  most important
backgrounds come from $ZZZ$, $ZZH$, and continuum $b\bar{b} q\bar{q}
q\bar{q}$ production.  The final selections correspond to efficiencies
of 36\%, 19\%, and 19\% for the charged lepton, neutrino, and quark
decay channels, respectively. 



Scaling the results from the $b\bar{b}b\bar{b}$ and $b\bar{b}WW$
analyses to the expected luminosity of 4~ab$^{-1}$,  the combination
of the 
varous channels yield a precision of 16.8\%  on the $HH$ total cross
section. 
Assuming the SM with only the Higgs self-coupling as a free parameter, 
this corresponds to an uncertainty of 27\% on that coupling.




At still higher energies,  vector boson fusion becomes the dominant  \hh
production channel.  In a linear collider, luminosity is expected to
increase linearly with $\sqrt{s}$ energy.   Thus, studies at 1~TeV assume a
data sample
of 8~ab$^{-1}$. It is shown in  \cite{Tian:2013qmi,KurataHHH} that the
\hh production cross section can readily be observed.  In the
same context of varying the trilinear Higgs coupling only, the 
Higgs self-coupling
can be determined to 10\%. 

The impact of the centre of mass energy on the trilinear Higgs coupling
measurement is studied by extrapolating the full simulation results done 
at 500~GeV and 1~TeV to other energies.  The extrapolation is done in
such as way as to take into account the dependence on $\sqrt{s}$ for both the
total cross sections and the interference contributions~\cite{TianHHH:2015}.
The results are shown in Fig.~\ref{fig:HHHSensitivity} as the blue
lines
for the two reactions. 
In addition to the results from realistic full simulations, the expectations for
the ideal case,  assuming no background and 100\% signal efficiency,
are shown as the red lines in the figure. The differences between the
blue and the red lines are large, a factor of 4--5.  This suggests that there is much room
for improvement
in the clustering algorithm used to identify
2-jet systems with the Higgs boson mass, which would 
lead to improvement in the final results.  Improvements could also come from better 
flavour-tagging algorithms and inclusion of additional  signal channels such as  
 $Z\to\tau^+\tau^-$. The figure does imply that $\sqrt{s}=500$--600 GeV is
 optimal for $e^+e^-\to ZHH$. On the other hand,
 $\sqrt{s}$ energies of  1~TeV or above would be needed for optimal
 measurement of
 $e^+e^-\to\nu\bar{\nu}HH$.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[tb]
  \centering
   \includegraphics[width=0.48\hsize]{HHFuture/fig/coupling_zhh_125_-1.pdf}
   \  \ 
    \includegraphics[width=0.48\hsize]{HHFuture/fig/coupling_nnhh_125_-1.pdf}  
  \caption{The expected precisions of
   $\lambda$ as a function of $\sqrt{s}$ for $e^+e^-\to ZHH$ ~(left) and
for $e^+e^-\to\nu\bar{\nu}HH$ ~(right). The two lines in each plot
correspond
to the ideal situation using Monte Carlo truth (red) and  the 
realistic situation (blue) using current full-simulation analyses.
The same integrated luminosities of 4~ab$^{-1}$ is 
assumed at all values of $\sqrt{s}$.}
  \label{fig:HHHSensitivity}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.75\hsize]{HHFuture/fig/precision_BSM_HHH.pdf}
  \caption{Expected precisions of $\lambda$ when $\lambda$ is enhanced
    or suppressed from its SM value.}
  \label{fig:HHHBSMresult}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Since large deviations of the  trilinear Higgs coupling are expected in some new physics 
models, 
it is interesting to see how the expected precisions would change in
that case.
Using the dependence of the cross section of the two reactions on the
Higgs self-coupling shown in Fig.~\ref{fig:HHHBSM}, we can  convert the
expected
precisions of the ILC measurements just described to  precisions on
the Higgs self-coupling at highly enhanced or suppressed values.
The results are shown in Fig.~\ref{fig:HHHBSMresult}.    The
two reactions, useful at 500 GeV and 1 TeV
respectively, are complementary in determining the trilinear Higgs coupling. 
If the trilinear Higgs coupling is indeed a factor of 2 larger, as
expected in models of electroweak baryogenesis 
described in Sec.~\ref{sec:cosmology},
the $ZHH$ process at 500~GeV is especially useful and 
would already provide 
a measurement with 15\% precision  on the enhanced value of the self-coupling. 



\section[$HH$ production at CLIC]{$HH$ --- CLIC \\ \contrib{P. Roloff, U. Schnoor}}
\label{sec:eedirectCLIC}

The
Compact Linear Collider (CLIC) is 
an $e^+e^-$ linear collider based on two-beam acceleration technology.   It is 
aimed
at precision studies of the Higgs boson, the top quark, and on
exploration for new physics in electroweak interactions.  CLIC is
planned to be constructed in three stages, the first at 380~GeV in the
centre of mass, the second at 1.5~TeV, and the third at 3~TeV.    CLIC
presented its conceptual design report in 2012~\cite{Aicheler:2012bya}.
A current update on the CLIC design and physics program can be found
in \cite{deBlas:2018mhx,Charles:2018vfv}.

In the CLIC program, the Higgs self-coupling would be studied at
the 1.5~TeV and 3~TeV stages.   The planned integrated 
luminosities for these stages are  2.5~ab$^{-1}$ and 5~ab$^{-1}$,
respectively, with 80\% polarization of the electron beam  and an
unpolarized
positron beam.   The luminosity is planned to be divided between the L
and R orientations at 80\%/20\%.   As in the ILC program, the CLIC
program of single Higgs measurements will produce values
of the Higgs branching fractions to the major decay modes to
sub-percent accuracy~\cite{Abramowicz:2016zbo,Robson:2018zje}.

The study \cite{Roloff:2019crr}  describes analyses 
of the $ZHH$ and $\nu\bar\nu HH$ reactions by the CLICdp group.  These
studies are based on full-simulation analyses with the \verb+CLIC_ILD+
detector model.  (In this  study, the second CLIC stage was taken
to be at 1.4~TeV.)   All relevant background processes are included in
simulation data.

The $\nu\bar\nu HH$ process is studied in the
$b\bar b b\bar b$ and $b\bar b W W^*$ Higgs decay channels.
The main background contributions originate from diboson production and $ZH$
production. A Boosted Decision Tree (BDT) is used to extract the
$\nu\bar\nu HH$  signal in the
dominant decay channel of \bbbb  production. The
measurement benefits
from the clean
collision environment of $e^+e^-$ linear colliders as well as the
excellent heavy flavour
tagging capabilities and the
accurate jet energy resolution realised in the CLIC detector model.

In the studies at 1.4~TeV, evidence for $\nu\bar\nu HH$ production is
found
with a significance of 3.6~$\sigma$, and the $ZHH$ process can be
observed at this stage with a significance of 5.9~$\sigma$.  In the
studies at 3~TeV with $e^-$ beam polarization,
 the $\nu\bar\nu HH$ reaction is observed already
with 700~fb$^{-1}$.  With the total integrated luminosity of
5~ab$^{-1}$, the  $\nu\bar\nu HH$ cross section can be measured with
a precision of 7.3\%, assuming that it takes the SM value.

The extraction of the Higgs self-coupling at CLIC is based on the
total cross section measurements, combined with information from the
differential cross
section to distinguish effects of the self-coupling diagram in
Fig.~\ref{fig:hhdiagrams}.   Because of the destructive interference
in the  $\nu\bar\nu HH$ process, there is an ambiguity in the
interpretation of the total cross section result, since, for the CLIC
beam polarizations, the cross
section for  $\lambda/\lambda_{SM} = 2.2$ is the same as that
predicted in the SM, see Fig.~\ref{fig:HHHBSM}. This ambiguity can be
resolved using the $ZHH$ measurement, but it is also resolved by
measuring the \hh invariant mass  distribution in the $\nu\bar\nu HH$ reaction.
Figure~\ref{mHHvary} shows how the measured shape of this distribution changes
as $\lambda/\lambda_{SM}$ is varied.   As $\lambda/\lambda_{SM}$
increases,   this mass distribution decreases noticeably in the region
$ 500 < m(HH) < 1000$~GeV while the peak of the distribution at
$m(HH)\sim 400$~GeV rises dramatically. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
  \centering
    \includegraphics[width=0.6\hsize]{HHFuture/fig/SumMj_Signals.pdf} 
    \vspace*{-0.2cm}
    \caption{\hh invariant mass distribution measured in CLIC
      full-simulation studies at 3~TeV for different values of Higgs
      self-coupling modifier $\kappa_{HHH} = \lambda/\lambda_{SM}$.
      The $WWHH$ coupling is held fixed at the SM value.   The
      simulation assumes 5~ab$^{-1}$ of data and the 80\%/20\%
                     division of polarization described in the
                             text~\cite{Roloff:2019crr}.}
  \label{mHHvary}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The value of  $\lambda/\lambda_{SM}$ can then be extracted from a
template fit
to the binned distribution of the invariant mass of the
reconstructed Higgs boson pair in bins of the BDT response.
This value can be combined with the result of the
$ZHH$ cross section measurement at 1.4~TeV  to
extract the value of the trilinear Higgs self-coupling and its uncertainties.
The resulting constraint that will be provided by the CLIC
measurements is found to be
\beq 
0.93  \leq \lambda/\lambda_{SM} \leq   1.11 \
\eeq{CLICvalue}
at the  68 \% C.L. 

 
\section{EFT interpretation of $HH$ measurements}
\label{sec:eedirectEFT}

Up to this point, we have considered only the situation in which 
$\lambda/\lambda_{SM}$, or the SMEFT parameter $c_6$, is free to vary
while the other possible EFT parameters are held fixed. This is
probably too stringent an assumption. A modification of the Higgs
sector that can give rise to a large change in the Higgs self-coupling
will probably also affect other SM couplings~\cite{Huang:2016cjm}.
These changes will independently lead to changes in the prediction for
the $HH$ production cross section.   A robust search for a
deviation in the Higgs self-coupling should take this into account.

We have discussed such a more general analysis for the process
 $gg\to \hh$ at hadron
colliders,
taking into account the possible variation of other SM parameters, in
Secs.~\ref{subsec:EFTtheory} and~\ref{sec:eft_fit_GPZ}.  We have shown that the
SMEFT can be used as a tool to quantify the influence of other
possible effects of new physics on the \hh production cross section,
and that, in principle at least, these effects can be controlled by
making a global fit to the SMEFT parameters. 

  A similar analysis has
been done  for the reaction $e^+e^-\to ZHH$ at
500~GeV~\cite{Barklow:2017awn}.  For the $e^+e^-$ analysis, it is
possible to include the effects of all relevant dimension-6 operators
that appear in the SMEFT.  When this is done,  it is seen that 
new physics effects different from the shift in the Higgs
self-coupling can potentially have a major influence on the \hh cross
section, easily swamping the variation due to $c_6$.
Fortunately, the high precision of single Higgs and other measurements
at an  $e^+e^-$ collider will allow these effects to be controlled.


%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.70\hsize]{HHFuture/fig/Zhhdiagrams.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Feynman diagrams contributing to $e^+e^-\to ZHH$ in the SMEFT
  with dimension-6 operators included.  The vertices shown are also
  typically
modified from their SM values by dimension-6 perturbations~\cite{Barklow:2017awn}.}
\label{fig:Zhhdiagrams}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The full set of diagrams contributing to $e^+e^-\to ZHH$ in the SMEFT at
tree level,
including SM vertices and all contributing dimension-6 operators, is shown
in Fig.~\ref{fig:Zhhdiagrams}.  One should note that, in general, the
vertices in these diagrams are not equal to the SM vertices but rather
include extra pieces due to the dimension-6 perturbations.

The
complete variation of the tree level cross section with the SMEFT coefficients is
given in \cite{Barklow:2017awn}.  Some of the smaller terms in the complete
expression are difficult to explain without reference to the
renormalization scheme used there. Here we will write  a simplified formula that gives the dependencies on the most important SMEFT coefficients.  We assume here the case of unpolarized beams.  Then
\beqa
\sigma/\sigma^{SM}(ZZH) &=& 1 + 0.56  c_6 + 4.15  c_H + 15.1 ( c_{WW})  \CR
&& +  62.1 (c_{HL} + c^\prime_{HL}) - 53.5 c_{HE} + \cdots \ .
\eeqa{UZhh}
The coefficients listed here come from the SMEFT Lagrangian terms
\beqa
\Delta {\cal L} &=& \frac{c_H}{2 v^2} \partial^\mu(\Phi^\dagger \Phi)
\partial_\mu(\Phi^\dagger \Phi) 
- \frac{ c_6\lambda}{v^2} (\Phi^\dagger \Phi)^3 
+ \frac{c_{WW}}{2v^2} \Phi^\dagger \Phi
W^a_{\mu\nu} W^{a\mu\nu} \CR 
& & + i \frac{c_{HL}}{v^2}  J_H^{\mu}  (\bar L
\gamma_\mu L)  + 4 i \frac{c'_{HL} }{ v^2}  J_H^{a \mu } (\bar L
\gamma_\mu t^a L) +  i \frac{c_{HE}}{ v^2} J_H^{\mu} (\bar e
\gamma_\mu e) \ ,
\eeqa{firstL}
where $W_{\mu\nu}^a$ is the SU(2) field strength, $L$ is the
left-handed lepton doublet $(\nu_e,e)_L$, and $J_H^\mu$, $J_H^{a\mu}$
are the Higgs currents $(\Phi^\dagger \Dlr{}^\mu \Phi)$ and
$(\Phi^\dagger t^a \Dlr{}^\mu \Phi)$, respectively.
In the full expression, the cross section depends on a total of 16
SMEFT coefficients at tree level.  Some of the numerical factors in Eq.~
\leqn{UZhh} are uncomfortably large.  And, unfortunately, because the phase
space for $e^+e^-\to ZHH$ is very restricted at 500~GeV and the cross
section is quite small, there is no useful additional information from
the differential distributions to separate the various dependencies.

However, it turns out that the accuracy of precision measurements at
$e^+e^-$ colliders is enough to solve the problem. The parameters
$c_{HL}$, $c'_{HL}$, $c_{HE}$ are tightly constrained by precision
electroweak measurements, even at the current LEP level of precision.
At a linear $e^+e^-$ collider, the parameters $c_H$ and $c_{WW}$ are
 constrained by the measurement of the total  cross
section for  $e^+e^-\to ZH$, the polarization asymmetry in this total
cross section, and the Higgs branching ratio to $WW^*$.  The analysis
\cite{Barklow:2017suo} describes a global fit to the data set that
will
be acquired in the ILC program with parameters that include the full
set of dimension-6 operators that contribute to the measured cross
sections at the tree level.   From the results of this analysis, it
is found that the expression in Eq.~\leqn{UZhh} can be evaluated with an
uncertainty of 2.8\% from the $c_H$ and $c_{WW}$ terms and
0.9\% from the $c_{HL}$, $c'_{HL}$, and $c_{HE}$ terms, and that these
errors are slightly correlated, so that the total uncertainty from
SMEFT coefficients other than $c_6$  (including those not
mentioned here)
is 2.4\%.   This gives a
systematic
error on the extraction of $c_6$ of 5\%, to be added in
quadrature to the
larger statistical error estimated in
Sec.~\ref{sec:eedirectILC}~\cite{Barklow:2017awn}.

It would be interesting to perform a similar analysis for the
measurements of the $\nu\bar\nu HH $ process. One difficulty to be
aware of it that the factors in front of the coefficients  $c_{HL}$,
$c'_{HL}$, and $c_{HE}$
grow as  $s/m_Z^2$.   However, these parameters can be controlled to
an even greater degree that was taken into account in
\cite{Barklow:2017awn} by the improvements in our knowledge of precision
electroweak observables that are expected from
 these $e^+e^-$ colliders~\cite{Benedikt:2018qee,Fujii:2019zll}.





\section{Indirect determination of the Higgs self-coupling ---  CEPC,
  FCCee, CLIC, ILC}
\label{sec:eeindirect}


The indirect determination of the trilinear Higgs self-coupling is based on
the observation of McCullough~\cite{McCullough:2013rea} that the cross
section for $e^+e^-\to ZH$ contains a radiative correction involving the
trilinear coupling that raises this  cross section by about 1.5\% in
the region of $\sqrt{s} \sim 250$~GeV. 
 Taken at face value in the simple context with only the
trilinear coupling free,  cross section measurements at an $e^+e^-$
Higgs factory at two different energies---for example,
the measurements from the ILC at 250 and
500~GeV---would determine the trilinear 
coupling to about 25\%.

Here, though, we are on even shakier ground in extracting a value of
the Higgs self-coupling without taking account of other possible SMEFT
effects on the Higgs production cross section. This is true for two
reasons.
First, as in the extraction
of the coupling from \hh production, there are many SMEFT effects
that could potentially influence the observables that we will use.
But in this case, some SMEFT effects shift these observables already
at the tree level, while the Higgs self-coupling enters as a loop
effect. Thus, even in a model in which the shift of most Higgs
couplings are at the few-percent level while the shift of the
self-coupling is at the order-1 level, the effects on the $ZH$ cross
section
will still be comparable in size.

%%%%%%%%%%%
\begin{figure}
\begin{center}
  \includegraphics[width=0.60\hsize]{HHFuture/fig/ZHH1loop.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Feynman diagrams contributing to the shift of the $ZHH$
  vertex due to the 1-loop effect of the Higgs self-coupling~\cite{McCullough:2013rea}.}
\label{fig:ZZH}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.70\hsize]{HHFuture/fig/McC.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Relative enhancement of the  $e^+e^-\to ZH$ cross section
  and the $h\to W^+W^-$ partial width, in \%,  for $\kappa_\lambda =
  1$, due to the 1-loop diagrams shown
  in Fig.~\ref{fig:ZZH}.   One $Z$ or $W$ leg is off-shell at the
  invariant $Q^2$ while the other $Z$ or $W$ and the Higgs boson are
  kept on-shell.  The vertical lines show the uncertainties expected
  from proposed $e^+e^-$ colliders from single measurements of the
  relevant
quantities,  green for FCC-ee, red for ILC.   For $Q> 200$~GeV, these
are 1~$\sigma$
error bars  for  measurements of
  $\sigma(e^+e^-\to ZH)$.  For $Q\sim 40$~GeV,  these are 
1~$\sigma$ errors on  $\Gamma(h\to WW^*)$, naively
  estimated as $\delta \Gamma = \delta BR(h\to WW^*)/(1-BR(WW^*)$. 
  Many more measurements are input to achieve the final values of the
  fit for $\kappa_\lambda$; see the text.}
\label{fig:McC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Fortunately, there is a feature that
can be used to separate the effect of the Higgs self-coupling from the
shifts of SMEFT coefficients representing other new physics effects.
The radiative correction highlighted by McCullough has a
characteristic dependence on the value of the $HWW$ and $HZZ$
couplings when one vector boson goes off-shell.  This effect is not
available for other Higgs couplings.  For example, at $e^+e^-$
colliders, the 
$Hb\bar b$, $Hgg$, and $H\tau^+\tau^-$ couplings are measured only
for the Higgs boson and the final-state particles on shell.
 (At a hadron collider,
the $hgg$ coupling can be measured for off-shell gluons using high-$p_T$ Higgs
production, but not to the sub-percent precision needed here.)
The $HWW$ and $HZZ$
couplings, however,  are measured at several different kinematic
points, 
corresponding to
the one-shell Higgs decays with one vector boson at $Q^2 \ll m_V^2$,
to the 
$e^+e^-\to ZH$ reaction, in which $Q^2 = s$, to  and $e^+e^-\to
\nu\bar\nu H$, 
in which the vector bosons are at spacelike momenta. 

The diagrams responsible for the influence of the Higgs self-coupling,
in Unitarity gauge, 
are shown in Fig.~\ref{fig:ZZH}.   The enhancements due to these
diagrams in
the $e^+e^-\to ZH$ cross section and the $h\to W^+W^-$ partial width
 are shown in Fig.~\ref{fig:McC} as a function of the 
off-shell momentum invariant $Q = \sqrt{Q^2}$ of one of the $Z$ boson
legs.   The other $Z$ boson and the Higgs boson  are held on shell. 
This function has a cusp
at the $ZH$ threshold.  The overall scale is a shift of order 1\%.
The SMEFT parameters $c_H$ and $c_{WW}$ can also affect these
observables at the 1\% level.   However, the effect of $c_H$ is
independent of $Q$ and the effect of $c_{WW}$ is approximately
proportional to $Q^2$.    Thus, a set of sufficiently accurate
measurements at
different values of $Q$ can single out this contribution.   The
expected accuracy of measurements at the ILC and the FCC-ee are shown
in the figure.   It is clear that the availability of cross section
measurements at two different centre-of-mass energies will  play an
essential role in the analysis. 

Most of the variation of the enhancement shown in Fig.~\ref{fig:McC}
takes place between the $ZH$ threshold and 350~GeV, so proposed linear
and circular $e^+e^-$ Higgs
factories compete here on a much more equal footing.   In addition to
ILC and CLIC discussed above, one should consider the  proposed Higgs
measurement programs of the Circular Electron-Positron Collider
(CEPC), proposed for construction in China, and the 
and the $e^+e^-$ stages of the Future Circular Collider (FCC-ee) proposed
for construction at CERN.    The CEPC conceptual design report was
presented in 2018~\cite{CEPCStudyGroup:2018rmc,CEPCStudyGroup:2018ghi}.
This report outlines a problem of  5.6~ab$^{-1}$ of data at 240~GeV,
plus an extensive program of precision electroweak measurements at the
$Z$ pole and $WW$ threshold.  A run at the $t\bar t$ threshold has
been studied, but it is not part of the proposed program at this
time.  The FCC-ee conceptual design report was
presented in
2019~\cite{Benedikt:2018qee}.   This report outlines a similar program
of precision electroweak and Higgs boson measurements up to 240~GeV
and also includes a run of 1.5~ab$^{-1}$  divided between 350~GeV and
365~GeV.

The effect of the Higgs self-coupling is visible but somewhat marginal
on the basis of the three observables shown in Fig.~\ref{fig:McC}.
However, this is only the starting point.   The fit for the
self-coupling from the indirect method becomes sharper when a larger
number of Higgs observables are included.  This is true even when the
fit contains the 16 SMEFT 
coefficients needed for a
complete accounting of the possible new physics corrections,  as in the analysis of
Sec.~\ref{sec:eedirectEFT}.   One should note that, in addition to
$c_H$ and $c_{WW}$, the
parameters $c_{HL}$, $c^\prime_{HL}$, and $c_{HE}$ in
Eq.~\ref{firstL} also have $Q^2$-dependent contributions.  However,
the measurement of 
precision electroweak and additional single-Higgs observables will
independently constrain these parameters.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\hsize]{HHFuture/fig/HFCplot.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Uncertainties on the Higgs self-coupling  projected for the
   High-Luminosity LHC and for other future colliders, at various
   stages,
   by the Higgs@Future Colliders working group~\cite{deBlas:2019rxi}.
   The results  are presented as uncertainties on  $\kappa_3 =
   \kappa_\lambda$. In the bar graphs, results from the direct method
   are shown with solid bars and result from the indirect method with
   hatched bars. The estimates for the indirect determination of
   the self-coupling are based on a multi-parameter SFEFT analysis
   which also takes into account projected results from the LHC.  (Estimates in parentheses correspond to a 1-parameter fit without other new physics effects.)
   The results for all $e^+e^-$ colliders include the projected
   indirect and direct
   results from the HL-LHC, approximated by a 50\% uncertaintly in
   $\kappa_\lambda$. }
\label{fig:HFC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


 
A full analysis using this strategy  has been carried out by the ECFA Higgs@Future
Colliders working group~\cite{deBlas:2019rxi}.  The results of this
analysis are shown in Fig.~\ref{fig:HFC} and given in tabular form in
Table~\ref{tab:future_comp} in the Summary  to Part III.  The latest
results on the precision electroweak capabilities of the various
$e^+e^-$ colliders are included.  The 
analysis by this group is made somewhat less transparent by the fact
that their analysis attempts to include improvements in the SMEFT
parameters that will come from the HL-LHC. 
All of the results from  the indirect method for future $e^+e^-$
colliders that are quoted in the figure and the table  are combined
with the uncertainty of approximately 50\%
expected from
the direct and indirect determinations of the Higgs self-coupling at
the HL-LHC.
Thus, only values significantly smaller than 50\%  show an 
improvement by the $e^+e^-$ data. Tthe only $e^+e^-$
results that achieve this are those from the  FCC-ee and ILC programs
with two energy stages.  As is  shown in Fig.~\ref{fig:McC},
the FCC-ee program features higher statistics
in the cross section measurements, but the ILC stage at 500~GeV offers
a somewhat longer moment arm, leading to comparable estimates of the
improvement when the full set of observables is taken into account. 

The FCC-ee group has considered a scheme with 4 IPs that offers higher
integrated luminosity at the high-energy
point~\cite{Blondel:2018aan}, which would achieve an uncertainty on
the self-coupling of about 30\% from $e^+e^-$ data alone or 24\% when
combined with HL-LHC.   Since the $e^+e^-$ results are
statistics-limited, improved results are possible in any scheme with
higher integrated luminosity at the point with higher $\sqrt{s}$,
either with additional detectors or with extended running time.  At
the moment, neither plan is included in the official FCC-ee proposal. 

Still, the planned ILC and FCC-ee programs  correspond to roughly  a
50\% uncertainty due to the  $e^+e^-$ data  alone.   This is
comparable to the expected precision from the HL-LHC direct
measurement. This indirect determination
would then provide a welcome independent measurement
of the self-coupling, and one that will be  essentially free of
model-dependent assumptions. 




\section{The quartic Higgs self-coupling}\label{sec_ee:quartic}

Up to this point in our discussion of $e^+e^-$ probes of the Higgs
potential, we have only considered dimension-6 operators in the
SMEFT.  For operators that specifically modify the Higgs potential, 
we have considered only one higher-dimension operator, the operator
with coefficient $c_6$ in Eq.~\leqn{lsmeft} whose main role is to
shift the coupling $\lambda_3$.   More general modifications of the
Higgs potential are available from operators of higher dimension.  It
is relevant to ask whether inclusion of this possibility affects the
determination of $c_6$ or $\lambda_3$.

This question was studied for the first time
in Ref.~\cite{Maltoni:2018ttu}.   This paper considered the
two-parameter  Higgs potential modification
\beq
   \Delta\mathcal{L} =  - \frac{\bar c_6}{v^2}\left(\Phi^\dagger\Phi - \frac{v^2}{ 2} \right)^3
 - \frac{\bar c_8}{v^4}\left(\Phi^\dagger \Phi- \frac{v^2}{ 2}\right)^4 \ ,
\eeq{sixeightL}
as in eq. \leqn{VNP},  including the dimension-6 and also a dimension-8 perturbation.  From
this effective Lagrangian one can define
\beqa
  c_6 &\equiv& (2 v^2/m_h^2) \bar c_6 \CR
  c_8 &\equiv& 4 (2 v^2/m_h^2) \bar c_8 \ .
  \eeqa{sixeightdefs}
Then, similarly to eq.~\leqn{eq:klrel},
\beqa
    \kappa_\lambda &\equiv& \frac{\lambda_3}{ \lambda_3^{SM}  } = 1 +
    c_6 \CR
   \kappa_4 &\equiv& \frac{\lambda_4 }{ \lambda_4^{SM}  } = 1 +
   6  c_6  +  c_8  \ .
\eeqa{kappasixeight}
In this context, it is possible to analyse processes with single Higgs
production, $HH$ production, and $HHH$ production to deduce
constraints on $c_6$ and $c_8$.  It is important to note that the
restriction of the fit to two possible operators is a simplification
with respet to the analyses described in the previous sections.   First,
$c_H$ and other possible dimension-6 operator coefficients
are  not
included in this analysis.  We have already seen in
Sec.~\ref{sec:eedirectEFT}, though, that 
the relevant operator coefficients would already be strongly constrained by 
expected measurements of single Higgs observables at $e^+e^-$
colliders.
But, further,  the effects of many more new operators appearing at dimension 8
are not included.   This  analysis assumes that  their coefficients are
suppressed
with respect to $c_8$.


The study of Ref.~\cite{Maltoni:2018ttu} derives constraints on these
two parameters by considering the deviations in the total cross
section for Higgs production processes at $e^+e^-$ colliders of
increasing energy, treating both $s$-channel $Z$ and $W$ fusion
reactions, and both  tree-level and one-loop effects of
the higher-dimension operators.    The specific processes considered,
and the loop order at which the two couplings first appear, are:
%are shown in the table:
\beq
\begin{tabular}{ccc}
Process &   $ \lambda_3$  & $\lambda_4$  \\ \hline
$ZH\ , \ \nu_e\bar\nu_e H$  &   one-loop  &  two-loop \\
$ZHH\ ,\ \nu_e\bar\nu_e HH$  &   tree  &  one-loop \\
$ZHHH\ ,\  \nu_e\bar\nu_e HHH$  &   tree  &   tree  \\
\end{tabular}
\eeq{eeHHprocesses}
In Ref.~\cite{Maltoni:2018ttu}, both tree and one-loop effects are
included for each process.   Two-loop corrections  are not included.
It is important to note that, while the one-loop effects on single Higgs
cross sections can be computed without reference to an underlying EFT
framework, the one-loop corrections to the $HH$ and $HHH$ cross sections are
UV-sensitive and require renormalization.  Using the  SMEFT formalism and taking advantage of the 
parametrization in eq.~\leqn{sixeightL}, the authors of 
Ref.~\cite{Maltoni:2018ttu} worked out these UV-finite expressions.

By changing the values of $c_6$ and $c_8$, one can
independently change the values of $\lambda_3$ and $\lambda_4$.   As
already noted, UV-finite radiative corrections due to $c_6$
and $c_8$  are taken into account.  
The analogous study for 
future hadron colliders, was first  presented in
Ref.~\cite{Borowka:2018pxx}.   This is technically more challenging
because of the need to consider two-loop calculations in the $gg$
fusion channel.   That analysis is described in Sec.~\ref{sec:other_probes}.

With this formalism in hand, Ref.~\cite{Maltoni:2018ttu} presented
constraints on the $ c_6$ and $c_8$ couplings that
would be obtained from the run programs of the proposed $e^+e^-$
colliders
CEPC, FCC-ee, ILC, and CLIC.   The strongest constraints apply to
ILC and CLIC at energies of 500~GeV and above, where \hh and
eventually $HHH$ production is observable.   In this case, we can
consider
the possibility that $c_8$ can be large and quote joint
constraints
on the two variables.   In particular, we can compare the allowed
range of $c_8$ to the theoretical limit 
$c_8\lesssim
31$ quoted in Eq.~\leqn{EFT:c8bound}.  A limitation of this strategy
is that the $HHH$ cross sections at $e^+e^-$ colliders are quite
small. The SM cross sections are shown in Fig.~\ref{fig:HHHcs}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.44\hsize]{HHFuture/fig/xs-vvhhh-nobar.pdf}\ \ 
\includegraphics[width=0.44\hsize]{HHFuture/fig/xs-zhhh-nobar.pdf}\ \ 
\end{center}
\vspace*{-0.4cm}
\caption{Leading order total cross sections for $ZHHH$ (left) and $W$ fusion
  $HHH$ (right)  in $e^+e^-$ collisions, for representative
  values of $c_6$ and $c_8$.  The red solid curves
  are the SM values.  The results refer to
  the ideal beam polarization choice  $P_{e^-} = -1.0$, $P_{e^+} = +1.0$.}
\label{fig:HHHcs}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-ilc-c6c8.pdf}\ 
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-clic-c6c8.pdf}\\ 
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-ilc-klk4.pdf}\ 
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-clic-klk4.pdf}
\end{center}
\vspace*{-0.5cm}
\caption{Combined 90\% CL constraints on the cubic and quadratic Higgs
  self-couplings from the $e^+e^-$ colliders ILC (left) and CLIC
  (right). 
 The upper plots show the 
constraints in the $(c_6, c_8)$ plane; the bottom
plots show the constraints in the $(\kappa_\lambda,\kappa_4)$ plane.
The red regions marked ILC-H and CLIC-H refer to a combination of all
single
 Higgs measurements at all energy stages for each collider under
 study.
 In all cases only the perturbative region described in
 Sec.~\ref{sec:theoretical_constraints_EFT}, $ |c_6| < 5$, $
 |c_8| < 31$,  has been considered. }
\label{fig:Pagani}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In Fig.~\ref{fig:Pagani},  we show as light and dark green regions the
90\% CL regions in this parameter space that would be obtained from
successive stages of running at ILC and CLIC from the measurements of 
$HH$ and $HHH$ production cross sections, assuming that the true
answer is the SM cross section.   The top plots show these 
constraints in the  $(c_6, c_8)$ plane; the bottom
plots show the constraints in the $(\kappa_\lambda,\kappa_4)$ plane.
For ILC, the analysis considers results from $ZHH$ production at
500~GeV  and its combination with results from $ZHHH$ and $W$ fusion
$HH(H)$ at 1~TeV.  (The relevant cross sections for $HHH$ production
are too small to be measured at 500~GeV.) For CLIC, the analysis
considers $ZHH(H)$ and $W$ fusion $HH(H)$ production at 1.4~TeV and 
3~TeV stages.   The luminosities and polarizations assumed are given
in Table~3 of \cite{Maltoni:2018ttu}; these differ in some details
from the current proposals in Refs.~\cite{Bambade:2019fyw} and \cite{Robson:2018enq}.
We also show as red bands the limits on $c_6$ from single
Higgs measurements at ILC and CLIC, using the indirect method
described in the Sec.~\ref{sec:eeindirect}, and assuming that the
two-loop dependence
on $c_8$  is negligible.   The 
CLIC constraints are stronger than ILC ones, thanks to the higher
energies and the greater accessibility of $HHH$ processes. On the
other hand, the $c_6$ constraints from single Higgs
production are stronger 
at the ILC.   Both this constraint and the measurement of $W$ fusion
at higher energies can be used to remove the two-fold ambiguity seen
in the plots for ILC500. Scenarios in which  the measured cross
sections differ from those of the SM have been investigated, assuming
that  they correspond to the more general case $|c_6| < 5$
and and $c_8 = 0$. For positive and large values of $c_6$, the constraints on both $c_6$ and $c_8$ 
become stronger than in the SM case, analogously to what we have already 
pointed out in the discussion of Fig.~\ref{fig:HHHBSMresult} for the case of $c_6$ only.

The conclusion of this study is that the first coarse bounds on the
value of 
$c_8$,   and in turn on $\lambda_4$, can be set at future
$e^+e^-$
 colliders. The SM rate for triple Higgs
production is not measurable at these $e^+e^-$ colliders, even at the
highest energies considered.  But the cross section strongly depends
on $\lambda_4$, and so it is possible to obtain significant constraints.  
The combination of results from double and triple Higgs production
at high energies improves the constraints.  The $W$ fusion channel
will give  the strongest bounds. For this reason, by increasing the
energy, the precision of the constraints on $\lambda_3$ and
$\lambda_4$ will improve, regardless of the true value of
$\lambda_3$.   
The constraints that can obtained at CLIC at 3~TeV via $W$ boson
fusion $HHH$ production are similar to those that should be obtained
 at a future 100~TeV hadron collider.



\section{Combination}

The conclusion of this section have now become clear:
\begin{itemize}
  \item  It is very difficult for an $e^+e^-$ collider operating at a
    single 
    energy below 500~GeV to place significant constraints on the Higgs
    self-coupling.
    \item An $e^+e^-$ collider with significant integrated luminosity at
      two different $\sqrt{s}$ energies (e.g., 250 and 350~GeV or 250 and
      500~GeV)  would be expected to measure the Higgs self-coupling
      to a precision of about 40
      \%.  This measurement would be
      model-independent, in the sense that it is insensitive to the
      values of other SMEFT coefficients that affect electroweak
      processes at the collider.
\item The ILC at 500~GeV would be expected to measure the Higgs
  self-coupling to 27\% by the direct measurement of \hh production.
    This measurement would be
      model-independent, in the sense that it is insensitive to the
      values of other SMEFT coefficients that affect electroweak
      processes at the collider.   The measurement could be combined
      with the indirect measurement  to produce a value of this
      coupling with an uncertainty of 22\%.
    \item The ILC at 1~TeV or CLIC in its proposed program at 1.5 and
      3~TeV would be expected to measure the Higgs self-coupling to
      about 10\% by 
      the direct measurement of \hh production  using the $ZHH$ and
      $\nu\bar\nu HH$ channels.   Though it is likely that this
      measurement would be model-independent, that needs further
      study.
    \item Both the ILC and CLIC programs would provide very strong
      evidence for an increase of the Higgs self-coupling by a factor
      of 2, as actually expected in models of electroweak
      baryogenesis.
    \end{itemize}

    There are reasons to guess that our knowledge of the Higgs
    self-coupling might be even better than that described here.
    First, all estimates from $e^+e^-$ colliders are based on current
    full-simulation analyses.   We have already pointed to large gaps
    between the results of these analyses and ideal analyses with
    perfect signal/background discrimination.   There is considerable
    room to be more clever when we are directly working with data.
    
    Second, these results from $e^+e^-$ colliders will be combined with
    results from $pp$ colliders operating in the same time frame.
     Hadron colliders can be very sensitive to $HH$ production, but there
     are clear difficulties seen today  in extracting model-independent
     estimates of the Higgs self-coupling.  This could be greatly
     assisted by the use of results from $e^+e^-$.   In particular, all
     four proposed Higgs factories are expected to constrain the
     parameter $c_{\Phi G}$ in Eq.~\leqn{lsmeft}, which contributes
     at the tree level in a SMEFT analysis of $gg\to HH$, by measuring
     the $Hgg$ coupling to 1\% precision~\cite{Bambade:2019fyw}.
     Feedback  between $e^+e^-$ and $pp$ measurements will eventually
      lead us to the most precise understanding of the Higgs self-coupling.
 

==> HHFuture/HHineev2.tex <==


\label{chap:ee}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}


\section{Introduction}

The  Higgs self-coupling can be measured at $e^+e^-$  colliders in two
different ways. First, the coupling can be measured using the $HH$
production processes $e^+e^-\to ZHH$   (double Higgsstrahlung) and
$e^+e^-\to \nu\bar\nu HH$ (vector boson fusion).  These are analogous
to the $HH$ production processes studied earlier in this report for
hadron colliders. 
Also, as at hadron colliders, the Higgs self-coupilng can be measured
using single-Higgs production processes.  Here, the use of $e^+e^-$ beams
offers two advantages.   First, $e^+e^-$  colliders promise an intrinsic precision in 
single-Higgs measurements that will be higher than at hadron colliders,
reaching or exceeding the 1\% level.   Second,  $e^+e^-$  colliders
offer a larger number of independent  single-Higgs observables that
can be used to great effect in the interpretation of the
measurements.

In this chapter, we will discuss all of these aspects in turn.   We
will set the stage in Sec.~\ref{sec:eescope}  by describing the proposed
next-generation $e^+e^-$ Higgs factories in terms of their expected
energies and integrated luminosities. All of these proposed
facilities---CEPC, FCC-ee, ILC, and CLIC---can carry out the
single-Higgs analysis, though only ILC and CLIC are expected to have a
sufficiently high CM energy to measure $HH$ production.
In Sec.~\ref{sec:oneHv1},
we will describe the capabilities of these facilities for
determining  the Higgs self-coupling through 
single-Higgs measurements.   The discussion here and in the next few
sections will be given in the simplest model context, in which a
variable $\kappa_\lambda$ is added to the SM and determined in a
1-parameter fit.

Sec.~\ref{sec:genHHee}  will discuss general
features of the $HH$ reactions available at $e^+e^-$ colliders.
Following this, we will review in Secs.~\ref{sec:eedirectILC} and
\ref{sec:eedirectCLIC} the analyses of $HH$ production reactions at
ILC and CLIC and the projected accuracy of the determination of
$\kappa_\lambda$.

In Secs.~\ref{sec:eedirectEFT} and \ref{sec:eeindirect}, we will
revisit these measurements in the context of the general description
of new physics effects by the SMEFT.    One should legitimately criticise
any projected accuracy in $\kappa_\lambda$  that is based on a
1-parameter fit.   Once we have determined that $\kappa_\lambda$ is
not equal to 1, we are in the domain of physics beyond the SM.   The
same new physics that alters $\kappa_\lambda$  can also, in principle,
alter the other couplings of the Higgs boson and, thus, can create
changes in measured single- and double-$H$ cross sections that have
nothing to do with the Higgs potential.    It turns out that $e^+e^-$
measurements offer incisive tools for separating the effect of
$\kappa_\lambda \neq 1$ from other new physics effects on the primary
observables.   Thus, in most cases, it is possible to determine the
magnitude of
$\kappa_\lambda$ specifically and to  separate its effects from those of
other, quite general, effects of new physics.
 We will present the analysis first, in
Sec.~\ref{sec:eedirectEFT}, for the determination from $HH$ production
and then, in Sec.~\ref{sec:eeindirect}, for the determination from
single-$H$ production.

Sec.~\ref{sec_ee:quartic}  will review a first attempt to determine
both the Higgs cubic and quartic couplings from $e^+e^-$ observables.
The analysis here will be given in a 2-parameter model that does not
include other possible new physics effects.   Finally,
Sec.~\ref{sec:eeconclude} will give some conclusions.


\section{Scope of the proposed $e^+e^-$ Higgs factories}
\label{sec:eescope}

At this time, four proposals for next-generation $e^+e^-$ colliders are
under consideration in different regions of the world.   Two of
these---the Circular Electron-Positron Collider (CEPC) and the Future
Circular (Lepton) Collider  (FCC-ee)--are large synchrotrons in tunnels of
circumference approximately 100~km. The other two---the International
Linear Collider (ILC) and the Compact Linear Collider (CLIC)---are single-pass
linear colliders.  The history of how these colliders came to be
proposed with different technologies in different regions is complex
and will not be explained here.  All four facilities have the same
basic goal, to provide precision measurements of the electroweak and
Higgs interactions at high energy and, in particular, to measure
parameters of the Higgs boson with better than 1\% precision.  The
measurements of $\kappa_\lambda$ and most other HIggs boson parameters
at $e^+e^-$ colliders are expected to be statistics-limited, so it is
important to pay attention to the sizes of the  total data sets
proposed for these machines.   The purpose of this section is to
provide a guide to the data sets currently proposed for the various
stages of each machine.

  The CEPC conceptual design report was
presented in 2018~\cite{CEPCStudyGroup:2018rmc,CEPCStudyGroup:2018ghi}.
This report outlines a program with 2 detectors  taking   5.6~ab$^{-1}$ of data at 240~GeV,
plus an extensive program of precision electroweak measurements at the
$Z$ pole and $WW$ threshold. These lower-energy stages have only
peripheral
importance for the determination of $\kappa_\lambda$.  A run at the $t\bar t$ threshold has
been studied, but it is not part of the proposed program at this
time.

 The FCC-ee conceptual design report was
presented in
2019~\cite{Benedikt:2018qee}.  The official accelerator parameters and
run schedule were also summarised in the report \cite{Bordry:2018gri}
on proposed future colliders at CERN.   The proposal for the FCC-ee
includes 2 detectors taking a total data set of  5~ab$^{-1}$  in a
first stage at 
240~GeV and
a data set of 1.5~~ab$^{-1}$  in a second stage
 divided between 350~GeV and
365~GeV.   In~\cite{Blondel:2018aan}, Blondel and Janot have proposed an
extended program  with 4 detectors, taking a total of 12~ab$^{-1}$ in
the 240~GeV stage and 5~ab$^{-1}$ at 350/365~GeV.   We will refer to
this scenario below as ``FCC-ee (4IP)''.   Similar improvements over
the FCC-ee proposal would be achieved with 2 detectors by doubling the
proposed running time.   This is quite feasible given the high
instantaneous luminosity of the machine.

The CLIC conceptual design report was presented in
2012~\cite{Aicheler:2012bya}.   An update of the design and run plan
was recently presented in  \cite{Charles:2018vfv} and the corresponding
physics case described in \cite{deBlas:2018mhx}.  The currently
proposed
accelerator parameters and
run schedule were also summarised in the report \cite{Bordry:2018gri}
on proposed future colliders at CERN. CLIC is planned to be
constructed in three stages, the first at 380~GeV with  1~ab$^{-1}$ of
integrated luminosity, the second at 1.5~TeV with 2.5~ab$^{-1}$, and
the third at 3~TeV with 5~ab$^{-1}$.


The ILC completed its technical design report in
2013~\cite{Behnke:2013xla}.
A recent review of the ILC
design and physics capabilities can be found in
\cite{Bambade:2019fyw}.   The ILC is planned to be constructed in two
stages, the first at 250~GeV  with  2~ab$^{-1}$ of
integrated luminosity, the second at 500~GeV  with 4~ab$^{-1}$, with an additional  short run at 350~GeV with 200~fb$^{-1}$.  The
current proposal for the ILC does not include a run at 1~TeV, but this
is within the capabilities of the ILC technology.  Parameters for 
1~TeV running were already given in the 2013 TDR.   The reports
\cite{Barklow:2015tja} and \cite{Bambade:2019fyw} describe a possible
run at 1~TeV taking 8~ab$^{-1}$ of data.   At this time, the MEXT
cabinet ministry in the Japan has expressed interest in the ILC and is
considering funding the first stage of the ILC as a part of the 2020 MEXT Master Plan.



\section{Determination of the Higgs self-coupling from single-Higgs
  reactions ---  CEPC,
  FCCee, CLIC, ILC}
\label{sec:oneHv1}

We first consider the determination of the trilinear Higgs
self-coupling from single-Higgs reactions.   The idea of this analysis
is similar to that presented in Sections~7.6 and 8.3.   If
$\kappa_\lambda \neq 1$, loop diagrams containing the triple-Higgs
vertex will produce radiative corrections to Higgs boson production
cross sections and decay rates that are proportional to
$\kappa_\lambda$.  These radiative
corrections are at the percent level.   Since $e^+e^-$ colliders are
designed to measure Higgs boson cross sections and branching ratios at
or below 
this level, their measurements can provide interesting constraints on
$\kappa_\lambda$.   The study of these constraints was initiated by
McCullough~\cite{McCullough:2013rea}, who pointed out that these
give a radiative correction that,
for $(\kappa_\lambda - 1)= 1$,
increases  the cross
section for $e^+e^-\to ZH$  by about 1.5\% at 
$\sqrt{s} \sim$~240--250~GeV.  Some more subtle aspects of
McCullough's analysis will be discussed in Sec.~\ref{sec:eeindirect}.

%%%%%%%%%%%
\begin{figure}
\begin{center}
  \includegraphics[width=0.60\hsize]{HHFuture/fig/ZHH1loop.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Feynman diagrams contributing to the shift of the $HZZ$
  vertex due to the 1-loop effect of the Higgs self-coupling~\cite{McCullough:2013rea}.}
\label{fig:ZZH}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


For $e^+e^-$ colliders, the most important such loop diagrams
are those shown in Fig.~\ref{fig:ZZH}.   These diagrams correct the
$HZZ$ vertex that appears in the production reaction $e^+e^-\to ZH$
and the decay $H\to ZZ^*$.   The very similar diagrams with external
$W$ bosons correct the
$HWW$ vertex that appears in the production reaction $e^+e^-\to
\nu\bar\nu H$
and the decay $H\to WW^*$.   The radiative correction to the $Ht\bar
t$ vertex, which contributes to the decay $h\to gg$ in 2 loops, gives
a smaller effect and will not be considered here.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\begin{center}
 \begin{tabular}{lcc}
collider  &   1-parameter  &  full SMEFT \\ \hline
CEPC 240 &         18\%            &       -         \\  \hline
FCC-ee 240 &       21\%         &        -         \\ 
FCC-ee 240/365 &     21\%         &    44\%       \\ 
FCC-ee (4IP)           &     15\%         &      27\%        \\ \hline
ILC 250          &       36\%               &        -        \\ 
ILC 250/500    &      32\%            &        58\%        \\  
ILC 250/500/1000 &      29\%           &     52\%       \\  \hline
CLIC 380           &          117\%         &         -         \\ 
CLIC 380/1500          &         72\%          &       -      \\ 
CLIC 380/1500/3000         &     49\%              &      -             \\ \hline
\end{tabular}
\end{center}
\vspace*{-0.3cm}
\caption{Uncertainties on the value of $\kappa_\lambda$ expected from
  precision measurements of single-Higgs observables at $e^+e^-$
  colliders, from ~\cite{deBlas:2019rxi}.  The collider scenarios are
  listed by name and CM energy.   More details on each can be found in
  Sec.~\ref{sec:eescope}.  An independent  uncertainty of 50\%
  from HL-LHC assumed in  \cite{deBlas:2019rxi} is removed here to
  clarify the $e^+e^-$ contribution.
 Results are given for a 1-parameter fit to the SM plus
  a varying $\kappa_\lambda$ and for a fit that includes the
  possibility of other new physics effects modelled by the
  SMEFT. Cases in which the SMEFT analysis does not close  are denoted 
  by ``-''.  The  physics of the SMEFT 
 analysis is described in Sec.~\ref{sec:eeindirect}.}
\label{tab:HFCfit}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Recently, the ECFA Higgs@Future Colliders working
group has performed fits to the expected set of single-Higgs
measurements to assess the sensitivity to deviations of the Higgs
self-coupling from its SM value~\cite{deBlas:2019rxi}.    These fits use the
 expected measurement accuracies for the various single Higgs
 observables
given in the references
cited  in the previous section.   The results are shown in
Table~\ref{tab:HFCfit}.   

 The table lists uncertainties from a
1-parameter fit, corresponding to the model in which the SM is
modified only by a shift of the parameter $\kappa_\lambda$,  and a fit
to a larger model including the most general new physics effects
parametrized by dimension-6 SMEFT operators.   The ECFA Higgs@Future
Colliders group has reported its results as combined with an expected
50\% uncertainty in $\kappa_\lambda$ expected from the HL-LHC.  To
clarify the extra information that will come from  $e^+e^-$
measurements,  the values given in the table remove the 
HL-LHC contribution and
quote results from $e^+e^-$ measurements alone.   In some cases of the
multi-parameter fit, the analysis does not close and the $e^+e^-$
results alone do not give a competitive constraint.   Those cases are
indicated in the Table by a ``-''.

In all cases, the 1-parameter analysis seems to indicate a substantial
sensitivity to the Higgs self-coupling.   Including the
possibility of other new physics effects weakens this sensitivity
substantially, but, for some scenarios, the constraint is still a
powerful one.  We will discuss the physics of the multi-parameter fit
 in Sec.~\ref{sec:eeindirect}.


\section{$HH$ production processes at $e^+e^-$ colliders}
\label{sec:genHHee}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.62\hsize]{HHFuture/fig/CrossSectionPlot.pdf}
\vspace*{-0.3cm}
\caption{Cross sections for the double Higgs production processes
  $e^+e^- \to ZHH$ and $e^+e^- \to \nu\bar{\nu}HH$, as a function of
  $\sqrt{s}$ for $m_H=125\,$GeV.   The cross sections are shown for
unpolarized beams.  These cross sections are higher -- in the latter
case, by almost a factor 2 -- when the $e^-$ beam is highly polarized
in the left-handed sense. } 
\label{fig:sigzhh_vvhh}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The cross sections for the $ZHH$ and $\nu\bar\nu HH$ production
processes at $e^+e^-$ colliders 
are shown in Fig.~\ref{fig:sigzhh_vvhh}.   The cross sections are
shown in this figure for unpolarized beams.   Planned analyses at
$e^+e^-$ colliders will make use of polarized beams.  Since the
$\nu\bar\nu HH$ process, in particular, requires the initial state
$e^-_Le^+_R$, working with polarized beams can raise the cross section
significantly, by almost a factor of 2.  Still, these cross sections
are very small, and the processes are difficult to recognize even in
the relatively clean environment of an $e^+e^-$ collider.

In both cases, the $HH$ production processes are multi-body reactions
whose
cross sections increase slowly from threshold.   Energies much higher
than the nominal threshold energies of 250~GeV and 341~GeV are need to
produce a significant event sample. 
 The $ZHH$ process  is thus not accessible at 350~GeV, but it 
can be studied at an $e^+e^-$ centre of mass (CM) energy of
500~GeV.   The $\nu\bar\nu HH$ reaction, which 
is a 4-body process, requires  still higher energies, optimally, CM
energies above 1~TeV.   The ILD group has
studied these reactions at CM energies of
500~GeV and 1~TeV~\cite{Tian:2013qmi, KurataHHH,Duerig:2016dvi}.    The
CLICdp group has studied these reactions at CM energies of 1.5~TeV and
3.0~TeV~\cite{Roloff:2019crr}.   We will describe the analyses
below.
In both cases, the
analyses are done in the framework of full simulation using detailed
detector models.   This simulation framework is reviewed in Secs.~6 and
7 of~\cite{Bambade:2019fyw}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.95\hsize]{HHFuture/fig/WWHH_feynman_diagrams.png}
\caption{Diagrams contributing to $e^+e^- \to \nu\bar{\nu}HH$.} 
\label{fig:hhdiagrams}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
The diagrams for both processes  include a diagram with
the Higgs self-coupling in interference with diagrams in which the two
Higgs bosons are radiated separately from $W$ or $Z$ propagators.  The
SM diagrams for $e^+e^-\to \nu\bar\nu HH$ are shown in Fig.~\ref{fig:hhdiagrams}.
Note that both processes appear at the tree level in the SM and, since
we are in the electroweak world, the tree level is a good
approximation to the full result.  

A remarkable feature of the $e^+e^-$ reactions is that the two
processes have opposite dependence on $\kappa_\lambda$.   That is, the 
self-coupling diagram interferes constructively with the other SM
diagrams in the case of $ZHH$ and destructively in the case of
$\nu\bar\nu HH$.   The dependence of the cross section on the  variation of
the Higgs self-coupling is shown in Fig.~\ref{fig:HHHBSM}.    This
means that, whatever the sign of the deviation of $\kappa_\lambda$
from 1, one of the two processes will have an increased cross section
and will thus have increased statistical sensitivity  to the actual value of
$\kappa_\lambda$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
  \centering
    \includegraphics[width=0.7\hsize]{HHFuture/fig/xsec_coupling_BSM.pdf} 
    \vspace*{-0.3cm}
    \caption{The dependence of the cross sections for \hh production as a
      function of the Higgs self-coupling $\lambda$ for
      $e^+e^-\to ZHH$ ~(red line) and for 
      $e^+e^-\to\nu\bar{\nu}HH$ ~(blue line).
      The values of  both $\lambda$ and $\sigma$ are scaled to their 
      SM values. Note that the exact results depend on the assumed beam
    polarizations, here taken in the ILC scheme.}
  \label{fig:HHHBSM}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Measurement of $HH$ production --- ILC}
\label{sec:eedirectILC}

The ILC in its second stage will have sufficient CM energy 
to observe the reaction $e^+e^-\to ZHH$. 
Full simulation studies show that discovery of this
double Higgsstrahlung process is possible within the planned program
of the ILC  with    4~ab$^{-1}$ of data at 500~GeV.  The run plan assumes polarisation of 80\% for the
electron beam and 30\% for the positron beam, with the beam
polarisations
divided  among LR/RL/LL/RR  polarisations as
40\%/40\%/10\%/10\%.  Using the ILD detector model in full-simulation
analyses, the ILD group studied the extraction of the $ZHH$ process
from background in the di-Higgs decay channels  $hh\to
b\bar{b}b\bar{b}$~\cite{Tian:2013qmi,Duerig:2016dvi} and $hh\to
b\bar{b}W^+W^-$~\cite{KurataHHH}.  At this point  in the ILC program,
the
absolute
branching ratios of the Higgs boson into the $b\bar b$ and $WW^*$
channels will already be known with sub-percent
accuracy~\cite{Bambade:2019fyw}.  The measurements of $\sigma\cdot BR$
for the two channels can then be applied directly to  determination of the $HH$
production cross section.  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.4\hsize]{HHFuture/fig/HmassforZHHlept.png}
  \quad
 \includegraphics[width=0.4\hsize]{HHFuture/fig/HmassforZHHhadr.png}
 \caption{Reconstruction of the Higgs boson mass in the measurements
  of the $e^+e^-\to ZHH$ cross section described in
\cite{Duerig:2016dvi}: left: highest energy Higgs boson in events
with $Z\to \ell^+\ell^-$; right: highest energy Higgs boson in
 events with  $Z\to q\bar q$. }
  \label{fig:eehmasses}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The measurement of the $ZHH$ cross section in the $b\bar{b}b\bar{b}$ mode
is described in detail in the Ph.D. thesis of
D\"urig~\cite{Duerig:2016dvi}.   She presents three  paralle1 analyses for
the channels of $Z$ decay to charged leptons, to neutrinos, and to
quarks (including $b\bar{b}$.  In each case, a kinematic fit is
carried out on the 4- or 6-jet system, and the output parameters from  this fit
are  supplied to multivariate classifiers. The reconstructed Higgs
masses in the cases of charged leptonic and hadronic $Z$ decays are
shown in Fig.~\ref{fig:eehmasses}.   The  most important
backgrounds come from $ZZZ$, $ZZH$, and continuum $b\bar{b} q\bar{q}
q\bar{q}$ production.  The final selections correspond to efficiencies
of 36\%, 19\%, and 19\% for the charged lepton, neutrino, and quark
decay channels, respectively. 



Scaling the results from the $b\bar{b}b\bar{b}$ and $b\bar{b}WW$
analyses to the expected luminosity of 4~ab$^{-1}$,  the combination
of the 
various channels yield a precision of 16.8\%  on the $HH$ total cross
section. 
Assuming a 1-parameter fit to  the SM with only the Higgs self-coupling as a free parameter, 
this corresponds to an uncertainty of 27\% on that coupling $\kappa_\lambda$.

At still higher energies,  vector boson fusion becomes the dominant  \hh
production channel.  In a linear collider, luminosity is expected to
increase linearly with CM energy.   Thus, studies at 1~TeV assume a
data sample
of 8~ab$^{-1}$~\cite{Bambade:2019fyw}.    It is shown in 
 \cite{Tian:2013qmi,KurataHHH} that the
$HH$  production cross section can readily be observed.  In the
same context of varying the trilinear Higgs coupling 
only,   $\kappa_\lambda$
can be determined to a precision of 10\%. 

The impact of the centre of mass energy on the trilinear Higgs coupling
measurement is studied by extrapolating the full simulation results done 
at 500~GeV and 1~TeV to other energies.  The extrapolation is done in
such as way as to take into account the dependence on $\sqrt{s}$ for both the
total cross sections and the interference contributions~\cite{TianHHH:2015}.
The results are shown in Fig.~\ref{fig:HHHSensitivity} as the blue
lines
for the two reactions. 
In addition to the results from realistic full simulations, the expectations for
the ideal case,  assuming no background and 100\% signal efficiency,
are shown as the red lines in the figure. The differences between the
blue and the red lines are large, a factor of 4--5.  This suggests that there is much room
for improvement
in the clustering algorithm used to identify
2-jet systems with the Higgs boson mass, which would 
lead to improvement in the final results.  Improvements could also come from better 
flavour-tagging algorithms and inclusion of additional  signal channels such as  
 $Z\to\tau^+\tau^-$. The figure does imply that $\sqrt{s}=500$--600 GeV is
 optimal for $e^+e^-\to ZHH$. On the other hand,
 $\sqrt{s}$ energies of  1~TeV or above would be needed for optimal
 measurement of
 $e^+e^-\to\nu\bar{\nu}HH$.

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[tb]
  \centering
   \includegraphics[width=0.48\hsize]{HHFuture/fig/coupling_zhh_125_-1.pdf}
   \  \ 
    \includegraphics[width=0.48\hsize]{HHFuture/fig/coupling_nnhh_125_-1.pdf}  
  \caption{The expected precisions of
   $\lambda$ as a function of $\sqrt{s}$ for $e^+e^-\to ZHH$ ~(left) and
for $e^+e^-\to\nu\bar{\nu}HH$ ~(right). The two lines in each plot
correspond
to the ideal situation using Monte Carlo truth (red) and  the 
realistic situation (blue) using current full-simulation analyses.
The same integrated luminosities of 4~ab$^{-1}$ is 
assumed at all values of $\sqrt{s}$.}
  \label{fig:HHHSensitivity}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[tb]
  \centering
  \includegraphics[width=0.67\hsize]{HHFuture/fig/precision_BSM_HHH.pdf}
  \caption{Expected precision of $\lambda$ when $\lambda$ is enhanced
    or suppressed from its SM value.}
  \label{fig:HHHBSMresult}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Since large deviations of the  trilinear Higgs coupling are expected in some new physics 
models, 
it is interesting to see how the expected precisions would change in
that case.
Using the dependence of the cross section of the two reactions on the
Higgs self-coupling shown in Fig.~\ref{fig:HHHBSM}, we can  convert the
expected
precisions of the ILC measurements just described to  precisions on
the Higgs self-coupling at highly enhanced or suppressed values.
The results are shown in Fig.~\ref{fig:HHHBSMresult}.    The
two reactions, useful at 500 GeV and 1 TeV
respectively, are complementary in determining the trilinear Higgs coupling. 
If the trilinear Higgs coupling is indeed a factor of 2 larger than
its SM value, as
expected in models of electroweak baryogenesis 
described in Sec.~\ref{sec:cosmology},
the $ZHH$ process at 500~GeV is especially useful and 
would already provide 
a measurement with 15\% precision  on the enhanced value of the self-coupling. 



\section[$HH$ production at CLIC]{Measurement of $HH$ production
 --- CLIC \\
 \contrib{P. Roloff, U. Schnoor}}
\label{sec:eedirectCLIC}


In the CLIC program, the Higgs self-coupling would be studied at
the 1.5~TeV and 3~TeV stages.   The planned integrated 
luminosities for these stages are  2.5~ab$^{-1}$ and 5~ab$^{-1}$,
respectively, with 80\% polarisation of the electron beam  and an
unpolarised
positron beam.   The luminosity is planned to be divided between the L
and R orientations at 80\%/20\%.   As in the ILC program, the CLIC
program of single Higgs measurements will produce values
of the Higgs branching fractions to the major decay modes to
sub-percent accuracy~\cite{Abramowicz:2016zbo,Robson:2018zje}.

The study \cite{Roloff:2019crr}  describes analyses 
of the $ZHH$ and $\nu\bar\nu HH$ reactions by the CLICdp group.  These
studies are based on full-simulation analyses with the \verb+CLIC_ILD+
detector model.  (In this  study, the second CLIC stage was taken
to be at 1.4~TeV.)   All relevant background processes are included in
simulation data.

The $\nu\bar\nu HH$ process is studied in the
$b\bar b b\bar b$ and $b\bar b W W^*$ Higgs decay channels.
The main background contributions originate from diboson production and $ZH$
production. A Boosted Decision Tree (BDT) is used to extract the
$\nu\bar\nu HH$  signal in the
dominant decay channel of \bbbb  production. The
measurement benefits
from the clean
collision environment of $e^+e^-$ linear colliders as well as the
excellent heavy flavour
tagging capabilities and the
accurate jet energy resolution realised in the CLIC detector model.

In the studies at 1.4~TeV, evidence for $\nu\bar\nu HH$ production is
found
with a significance of 3.6~$\sigma$, and the $ZHH$ process can be
observed at this stage with a significance of 5.9~$\sigma$.  In the
studies at 3~TeV with $e^-$ beam polarisation,
 the $\nu\bar\nu HH$ reaction is observed already
with 700~fb$^{-1}$.  With the total integrated luminosity of
5~ab$^{-1}$, the  $\nu\bar\nu HH$ cross section can be measured with
a precision of 7.3\%, assuming that it takes the SM value.

The extraction of the Higgs self-coupling at CLIC is based on the
total cross section measurements, combined with information from the
differential cross
section to distinguish effects of the self-coupling diagram in
Fig.~\ref{fig:hhdiagrams}.   Because of the destructive interference
in the  $\nu\bar\nu HH$ process, there is an ambiguity in the
interpretation of the total cross section result, since the cross
section for  $\lambda/\lambda_{SM} = 2.2$ is the same as that
predicted in the SM, see Fig.~\ref{fig:HHHBSM}. This ambiguity can be
resolved using the $ZHH$ measurement, but it is also resolved by
measuring the \hh invariant mass  distribution in the $\nu\bar\nu HH$ reaction.
Figure~\ref{mHHvary} shows how the measured shape of this distribution changes
as $\lambda/\lambda_{SM}$ is varied.   As $\lambda/\lambda_{SM}$
increases,   this mass distribution decreases noticeably in the region
$ 500 < m(HH) < 1000$~GeV while the peak of the distribution at
$m(HH)\sim 400$~GeV rises dramatically. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]
  \centering
    \includegraphics[width=0.6\hsize]{HHFuture/fig/SumMj_Signals.pdf} 
    \vspace*{-0.2cm}
    \caption{\hh invariant mass distribution measured in CLIC
      full-simulation studies at 3~TeV for different values of Higgs
      self-coupling modifier $\kappa_{HHH} = \lambda/\lambda_{SM}$.
      The $WWHH$ coupling is held fixed at the SM value.   The
      simulation assumes 5~ab$^{-1}$ of data and the 80\%/20\%
                     division of polarisation described in the
                             text~\cite{Roloff:2019crr}.}
  \label{mHHvary}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The value of  $\lambda/\lambda_{SM}$ can then be extracted from a
template fit
to the binned distribution of the invariant mass of the
reconstructed Higgs boson pair in bins of the BDT response.
This value can be combined with the result of the
$ZHH$ cross section measurement at 1.4~TeV  to
extract the value of the trilinear Higgs self-coupling and its uncertainties.
The resulting constraint that will be provided by the CLIC
measurements is found to be
\beq 
0.93  \leq \lambda/\lambda_{SM} \leq   1.11 \
\eeq{CLICvalue}
at the  68 \% C.L. 

 
\section{SMEFT interpretation of $HH$ measurements}
\label{sec:eedirectEFT}

Up to this point, we have considered $HH$ production only using the
model in which 
$\kappa_\lambda = \lambda/\lambda_{SM}$ is free to vary
while the other possible new physics effects have been ignored. This is
probably too stringent an assumption. A modification of the Higgs
sector that can give rise to a large change in the Higgs self-coupling
will probably also affect other SM couplings~\cite{Huang:2016cjm}.
These changes will independently lead to changes in the prediction for
the $HH$ production cross section.   A robust search for a
deviation in the Higgs self-coupling should take this into account.

%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.8\hsize]{HHFuture/fig/Huang.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Parameter scan of the models considered in
  \cite{Huang:2016cjm}, showing the values of the $HHH$ and $HZZ$
  couplings relative to the SM prediction.   The colors indicate the
  strength of the first-order electroweak phase  transition in each model.
  We caution the reader that the grey lines indicated 
  projected measurements for future colliders should be 
  ignored; these estimates from 2016 are 
  superseded by more current ones presented in 
  \cite{Cepeda:2019klc} and the reports cited in Sec.~\ref{sec:eescope}.}
\label{fig:eeHuang}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


An example of this effect of new physics is shown in
Fig.~\ref{fig:eeHuang}.  This figure refers to a class of models in
which the Higgs self-coupling is modified through mixing with a SM
singlet scalar field.  This is a subset of the models considered in
Sec.~\ref{sec:BSMspin0}, without separately observable scalar resonances.
These models can still  generate a large shift in
the Higgs self-coupling to produce a first-order electroweak phase transition
as required for successful electroweak
baryogenesis.  This mechanism also generates smaller tree-level shifts in
the $HWW$ and $HZZ$ couplings.   As the figure shows, some models in
this class generate shifts of the single-Higgs couplings visible at
the HL-LHC, while other models produce smaller effects, requiring the higher precision available
at  $e^+e^-$ colliders for their observation.  These modifications of the
Higgs boson couplings to vector bosons will modify the SM predictions
for the $HH$ production cross sections in a manner that is independent
of the modification generated by a shift in $\kappa_\lambda$.  
To claim a measurement of $\kappa_\lambda$, the  influence of the
altered $HVV$ couplings must be  separated out.
  
In
Secs.~\ref{subsec:EFTtheory} and~\ref{sec:eft_fit_GPZ}, we have 
discussed such a more general analysis for the process
 $gg\to \hh$ at hadron
colliders.  We described using the SMEFT to take into account possible
new physics effects on the $HH$ production cross section that are
independent of changes in the Higgs self-coupling. We have shown that the
SMEFT can be used as a tool to quantify the influence of these
orthogonal effects of new physics
and that, in principle at least, these effects can be controlled by
making a global fit to the SMEFT parameters. 

  A similar analysis has
been carried out  for the reaction $e^+e^-\to ZHH$ at
500~GeV~\cite{Barklow:2017awn}.  Because the $e^+e^-$ cross section
depends on fewer operators than the cross section at hadron colliders,
it is 
possible to include the effects of all relevant dimension-6 operators
that appear in the SMEFT.  When this is done,  it is seen that 
new physics effects different from the shift in the Higgs
self-coupling can potentially have a major influence on the $HH$  cross
section, easily swamping the variation due to $\kappa_\lambda$.
Fortunately, the high precision expected for  single Higgs and other measurements
at an  $e^+e^-$ collider will allow these effects to be controlled.


%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.70\hsize]{HHFuture/fig/Zhhdiagrams.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Feynman diagrams contributing to $e^+e^-\to ZHH$ in the SMEFT
  with dimension-6 operators included.  The vertices shown are also
  typically
modified from their SM values by dimension-6 perturbations~\cite{Barklow:2017awn}.}
\label{fig:Zhhdiagrams}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The full set of diagrams contributing to $e^+e^-\to ZHH$ in the SMEFT at
tree level,
including SM vertices and all contributing dimension-6 operators, is shown
in Fig.~\ref{fig:Zhhdiagrams}.  One should note that, in general, the
vertices in these diagrams are not equal to the SM vertices but rather
include extra pieces due to the dimension-6 perturbations.

The
complete variation of the tree level cross section with the SMEFT coefficients is
given in \cite{Barklow:2017awn}.  Some of the smaller terms in the complete
expression are difficult to explain without reference to the
renormalisation scheme used there. Here we will write  a simplified
formula that gives the dependencies on the most important SMEFT
coefficients.  We assume here the case of unpolarised beams. 
In the SMEFT, $\kappa_\lambda$ receives two different contributions
from 
coefficients of dimension-6 operators.  In particular, we saw in
Eq.~\leqn{eq:klrel} that
 \beq
 \kappa_\lambda = 1 +  c_6  - \frac{3}{2} c_H \ , 
 \eeq{recallklrel}
where the parameter $c_6$ is the coefficient of an operator that
modifies the Higgs potential and  $c_H$ is a universal rescaling of all Higgs
 couplings that originates from a modification of the Higgs field
 kinetic term.   When we speak of a new physics modification of the
 Higgs potential within the SMEFT, we are speaking specifically about
 the generation of a nonzero value for $c_6$.

In terms of these two parameters and other coefficients of electroweak
dimension-6 operators, the ratio of the unpolarised total 
 cross section  for $e^+e^-\to ZHH$ at 500~GeV to its SM value 
is given at the tree level  by the expression
\beqa
\sigma/\sigma^{SM}(ZHH) &=& 1 + 0.56  c_6 - 4.15  c_H + 15.1 ( c_{WW})  \CR
&& +  62.1 (c_{HL} + c^\prime_{HL}) - 53.5 c_{HE} + \cdots \ ,
\eeqa{UZhh}
where the omitted terms are less important.
The coefficients listed here come from the SMEFT Lagrangian terms
\beqa
\Delta {\cal L} &=& \frac{c_H}{2 v^2} \partial^\mu(\Phi^\dagger \Phi)
\partial_\mu(\Phi^\dagger \Phi) 
- \frac{ c_6\lambda}{v^2} (\Phi^\dagger \Phi)^3 
+ \frac{c_{WW}}{2v^2} \Phi^\dagger \Phi
W^a_{\mu\nu} W^{a\mu\nu} \CR 
& & + i \frac{c_{HL}}{v^2}  J_H^{\mu}  (\bar L
\gamma_\mu L)  + 4 i \frac{c'_{HL} }{ v^2}  J_H^{a \mu } (\bar L
\gamma_\mu t^a L) +  i \frac{c_{HE}}{ v^2} J_H^{\mu} (\bar e
\gamma_\mu e) \ ,
\eeqa{firstL}
where $W_{\mu\nu}^a$ is the SU(2) field strength, $L$ is the
left-handed lepton doublet $(\nu_e,e)_L$, and $J_H^\mu$, $J_H^{a\mu}$
are the Higgs currents $(\Phi^\dagger \Dlr{}^\mu \Phi)$ and
$(\Phi^\dagger t^a \Dlr{}^\mu \Phi)$, respectively.
In the full expression, the cross section depends on a total of 17
SMEFT coefficients.  Some of the numerical factors in Eq.~\leqn{UZhh} 
are uncomfortably large.  And, unfortunately, because the phase
space for $e^+e^-\to ZHH$ is very restricted at 500~GeV and the cross
section is quite small, there is no useful additional information from
the differential distributions to separate the various dependencies.

However, it turns out that the accuracy of precision measurements at
$e^+e^-$ colliders is enough to solve the problem. The parameters
$c_{HL}$, $c'_{HL}$, $c_{HE}$ are tightly constrained by precision
electroweak measurements, even at the current LEP level of precision.
At a linear $e^+e^-$ collider, the parameters $c_H$ and $c_{WW}$ are
 constrained by the measurement of the total  cross
section for  $e^+e^-\to ZH$, the polarisation asymmetry in this total
cross section, and the Higgs branching ratio to $WW^*$.  The analysis
\cite{Barklow:2017suo} describes a global fit to the data set that
will
be acquired in the ILC program.  The  parameters in this fit include the full
set of dimension-6 operators that contribute to the measured cross
sections at the tree level.   From the results of this analysis, it
is found that, apart from the $c_6$ term, 
 the expression in Eq.~\leqn{UZhh} can be evaluated with an
uncertainty of 2.8\% from the $c_H$ and $c_{WW}$ terms and
0.9\% from the $c_{HL}$, $c'_{HL}$, and $c_{HE}$ terms.  These
errors are slightly correlated, so the total uncertainty from
SMEFT coefficients other than $c_6$  (including those not
mentioned here)
is 2.4\%.   This gives a
systematic
error on the extraction of $c_6$ of 5\%, to be added in
quadrature to the
larger statistical error estimated in
Sec.~\ref{sec:eedirectILC}~\cite{Barklow:2017awn}.  In many of the
models shown in Fig.~\ref{fig:eeHuang}, the value of $c_{WW}$ is 
large enough that it makes a significant correction to the value of
the $HH$ production cross section.  Nevertheless, this correction will
be known from the   single-Higgs data and can be subtracted without
loss of accuracy in the determination of $c_6$. 



 With the
contributions from these additional dimension-6 operator coefficients
under control, the measurement of the total cross section for the
reaction $e^+e^-\to ZHH$ can be interpreted as a model-independent 
measurement of $c_6$ within the broad class of models describable by
the SMEFT. 


It would be interesting to perform a similar analysis for the
measurements of the $\nu\bar\nu HH $ process. One difficulty to be
aware of it that the factors in front of the coefficients  $c_{HL}$,
$c'_{HL}$, and $c_{HE}$
grow as  $s/m_Z^2$.   However, these parameters can be controlled to
an even greater degree than was taken into account in
\cite{Barklow:2017awn} by the improvements in our knowledge of precision
electroweak observables that are expected from
 these $e^+e^-$ colliders~\cite{Benedikt:2018qee,Fujii:2019zll}.




\section{SMEFT interpretation of single-Higgs reaction 
measurements}
\label{sec:eeindirect}


Just as for the $HH$ determination of the Higgs self-coupling, it is
important to ask whether the determination of the self-coupling from
single-Higgs measurements can be affected by other new physics
contributions.  Here again we can use the SMEFT to quantify these
effects and eventually to separate them from the effects of the
self-coupling. 

However, there is an important difference between the situation for
the single-Higgs determination and that described in the previous
section.    In Eq.~\leqn{UZhh}, the contributions from all of the
SMEFT parameters appeared with numerical coefficients of order 1.
However, for the corresponding expressions in the 
single-Higgs case, while  most of the SMEFT parameters
enter with order-1 coefficients, the contribution from $c_6$ which we
are most interested in has a coefficient of order 1\%.   This is
expected, since most of the relevant SMEFT operators enter these
formulae at the tree-level, while $c_6$ enters only at the 1-loop
level.  For example, for the ratio of the unpolarized cross section
for $e^+e^-\to ZH$ at 250~GeV, the formula corresponding to Eq.~\leqn{UZhh}
is
\beqa
\sigma/\sigma^{SM}(ZH) &=& 1 + 0.015  c_6 -  c_H + 4.7 ( c_{WW})  \CR
&& +  13.9 (c_{HL} + c^\prime_{HL}) - 12.1 c_{HE} + \cdots \ .
\eeqa{UZoneh}
Thus, very strong constraints are needed on all of the additional
variables in Eq.~\leqn{UZoneh} to extract any information about
$c_6$. 



%%%%%%%%%%%
\begin{figure}
\begin{center}
\includegraphics[width=0.70\hsize]{HHFuture/fig/McCv2.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Relative enhancement of the  $e^+e^-\to ZH$ cross section
  and the $h\to W^+W^-$ partial width, in \%,  for $\kappa_\lambda =
  1$, due to the 1-loop diagrams shown
  in Fig.~\ref{fig:ZZH}.   One $Z$ or $W$ leg is off-shell at the
  invariant $Q^2$ while the other $Z$ or $W$ and the Higgs boson are
  kept on-shell.  The vertical lines show the uncertainties expected
  from proposed $e^+e^-$ colliders from single measurements of the
  relevant
quantities,  green for FCC-ee, red for ILC.   For $Q> 200$~GeV, these
are 1~$\sigma$
error bars  for  measurements of
  $\sigma(e^+e^-\to ZH)$.  For $Q\sim 40$~GeV,  these are 
1~$\sigma$ errors on  $\Gamma(h\to WW^*)$ from the SMEFT fits to the
full collider programs for FCC-ee and ILC reported
in \cite{deBlas:2019rxi}.}
\label{fig:McC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In \cite{DiVita:2017vrr}, Di Vita and collaborators explained that the expected
accuracy of single-Higgs measurements at $e^+e^-$ colliders will be
such that it is feasible to extract a value of $c_6$ despite this
difficulty.   They noted, in particular, that the enhancement of the
$HZZ$ and $HWW$ couplings highlighted by McCullough and discussed in 
Sec.~\ref{sec:oneHv1} has a special feature that aids this process.   
This radiative correction arises from the Feynman diagrams shown in
Fig.~\ref{fig:ZZH}.
It is useful to consider these diagrams as being evaluated with the
Higgs boson and one $Z$ or $W$ boson on mass shell while the other
vector boson is off-shell at a variable momentum invariant $Q = \sqrt{Q^2}$.
The value of the sum of diagrams has a characteristic dependence on
$Q$ that cannot be reproduced as a sum of effects of pointlike
dimension-6 SMWFT operators.   This is shown in Fig.~\ref{fig:McC}.
The diagrams give an enhancement that is not monotonic as a function of
$Q$ but rather has a sharp cusp at the $ZH$ threshold  ($Q = m_H
+ m_Z$).   Measurements at $e^+e^-$ Higgs factories will measure
this function at several different values of $Q$:  at values of $Q$
equal to the CM energies at the various collider
stages in the cross section $\sigma(e^+e^-\to ZH)$, at $Q \sim 40$~GeV
in 
the partial width $\Gamma(H\to WW^*)$,  at
 $Q \sim 30$~GeV in the partial width $\Gamma(H\to ZZ^*)$, and at $Q^2 \lesssim
0$
in the vector boson fusion cross section  $\sigma(e^+e^- \to \nu\bar\nu H)$.
Fig.~\ref{fig:McC} shows the expected accuracy of the three most
important of these measurements in the FCC-ee and ILC programs and
indicates how the set of three measurements can provide independent
values for the SMEFT parameters $c_6$, $c_H$, and $c_{WW}$.

Some caution should be used in interpreting this plot directly.  The errors
shown for $\Gamma(H\to WW^*)$ are those from the SMEFT fits done in 
\cite{deBlas:2019rxi} using the expected results from the full
FCC-ee and ILC programs.  Thus, they use the values of the indicated
cross section plus other data.   A full SMEFT analysis would include
many other measurements than the three indicated here, including
other measurements that put powerful constraints on $c_{WW}$.  On the
other hand, such an analysis would be based on  17 SMEFT parameters,
not just the few indicated in Eq.~\leqn{UZoneh}. 

The analysis that we have described does not include possible loop
corrections to the other Higgs couplings, for example, the influence
of the 
loop corrections to the $Hbb$ vertex or the $Htt$ vertex on
$\Gamma(H\to gg)$. 
In these cases, however, the vertex is measured only at one value of
$Q$, so the effect of $c_6$ is indistinguishable from a simple
$Q$-independent shift of the coupling strength, which is controlled by
a separate SMEFT parameter.   So, actually, only the corrections to
the $HZZ$ and $HWW$ couplings give sensitivity to $c_6$. 

A complete fit of the SMEFT parameters to the expected single-Higgs
data from the proposed Higgs factories has recently been carried out
by the ECFA Higgs@Future Colliders working
group~\cite{deBlas:2019rxi}.   The results of this analysis for the
projected uncertainty in $c_6$ are shown in Fig.~\ref{fig:HFC}.  The
results are those shown in the second column of
Table~\ref{tab:HFCfit},
except that the numbers in the figure are combined with an expected 50\%
uncertainty on $c_6$ from the measurement  of the $HH$
production cross section at tht HL-LHC. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\hsize]{HHFuture/fig/HFCplot.pdf}
\end{center}
\vspace*{-0.3cm}
\caption{Uncertainties on the Higgs self-coupling  projected for the
   High-Luminosity LHC and for other future colliders, at various
   stages,
   by the ECFA Higgs@Future Colliders working group~\cite{deBlas:2019rxi}.
   The results  are presented as uncertainties on  $\kappa_3 =
   \kappa_\lambda$. In the bar graphs, results from the direct method
   are shown with solid bars and result from the indirect method with
   hatched bars. The estimates for the indirect determination of
   the self-coupling are based on a multi-parameter SFEFT analysis
   which also takes into account projected results from the LHC.  (Estimates in parentheses correspond to a 1-parameter fit without other new physics effects.)
   The results for all $e^+e^-$ colliders include the projected
   indirect and direct
   results from the HL-LHC, approximated by a 50\% uncertainty in
   $\kappa_\lambda$. }
\label{fig:HFC}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The results in Fig.~\ref{fig:HFC} and Table~\ref{tab:HFCfit} show that
it is very important for the closure of the 17-parameter fit to have
data on $e^+e^-\to ZH$ at two different CM energies.  The cross
section for this reaction falls off rapidly at energies above 250~GeV,
so the plan of the FCC-ee to take data at 250~GeV and 365 GeV is more
optimal from this perspective.  For ILC, there is some compensation in
that the function shown in Fig.~\ref{fig:McC} has a larger variation
with $Q$ from 250~GeV to 500~GeV.   For CLIC, though running above
1~TeV allows the excellent measurements of $HH$ production described
above, the $ZH$ process is well measured only at the 380~GeV stage and
so $c_6$ is poorly constrained by the single-Higgs analysis. 

Finally, though, the FCC-ee and ILC programs would be expected to
yield a measurement of $c_6$ from single-Higgs processes with an
uncertainty of  40--60\%, independently of any results from $HH$
production.  This is
comparable to the expected precision from the HL-LHC.
This indirect determination
would then provide a welcome independent measurement
of the self-coupling. This measurement is expected to be statistics-limited and so would benefit from an increase in the running time or, in the case of circular machines, doubling the number of detectors.  We emphasise again that this measurement is  essentially free of
model-dependent assumptions within the broad class of models that can
be described by the SMEFT.  




\section{The quartic Higgs self-coupling}\label{sec_ee:quartic}

Up to this point in our discussion of $e^+e^-$ probes of the Higgs
potential, we have only considered dimension-6 operators in the
SMEFT.  For operators that specifically modify the Higgs potential, 
we have considered only one higher-dimension operator, the operator
with coefficient $c_6$ in Eq.~\leqn{lsmeft} whose main role is to
shift the coupling $\lambda_3$.   More general modifications of the
Higgs potential are available from operators of higher dimension.  It
is relevant to ask whether inclusion of this possibility affects the
determination of $c_6$ or $\lambda_3$.

This question was studied for the first time
in Ref.~\cite{Maltoni:2018ttu}.   This paper considered the
two-parameter  Higgs potential modification
\beq
   \Delta\mathcal{L} =  - \frac{\bar c_6}{v^2}\left(\Phi^\dagger\Phi - \frac{v^2}{ 2} \right)^3
 - \frac{\bar c_8}{v^4}\left(\Phi^\dagger \Phi- \frac{v^2}{ 2}\right)^4 \ ,
\eeq{sixeightL}
as in eq. \leqn{VNP},  including the dimension-6 and also a dimension-8 perturbation.  From
this effective Lagrangian one can define
\beqa
  c_6 &\equiv& (2 v^2/m_h^2) \bar c_6 \CR
  c_8 &\equiv& 4 (2 v^2/m_h^2) \bar c_8 \ .
  \eeqa{sixeightdefs}
Then, similarly to eq.~\leqn{eq:klrel},
\beqa
    \kappa_\lambda &\equiv& \frac{\lambda_3}{ \lambda_3^{SM}  } = 1 +
    c_6 \CR
   \kappa_4 &\equiv& \frac{\lambda_4 }{ \lambda_4^{SM}  } = 1 +
   6  c_6  +  c_8  \ .
\eeqa{kappasixeight}
In this context, it is possible to analyse processes with single Higgs
production, $HH$ production, and $HHH$ production to deduce
constraints on $c_6$ and $c_8$.  It is important to note that the
restriction of the fit to two possible operators is a simplification
with respect to the analyses described in the previous sections.   First,
$c_H$ and other possible dimension-6 operator coefficients
are  not
included in this analysis.  We have already seen in
Sec.~\ref{sec:eedirectEFT}, though, that 
the relevant operator coefficients would already be strongly constrained by 
expected measurements of single Higgs observables at $e^+e^-$
colliders.
But, further,  the effects of many more new operators appearing at dimension 8
are not included.   This  analysis assumes that  their coefficients are
suppressed
with respect to $c_8$.  Nevertheless, this analysis represents a first
step toward answering this question.


The study of Ref.~\cite{Maltoni:2018ttu} derives constraints on these
two parameters by considering the deviations in the total cross
section for Higgs production processes at $e^+e^-$ colliders of
increasing energy, treating both $s$-channel $Z$ and $W$ fusion
reactions, and both  tree-level and one-loop effects of
the higher-dimension operators.    The specific processes considered,
and the loop order at which the two couplings first appear, are:
%are shown in the table:
\beq
\begin{tabular}{ccc}
Process &   $ \lambda_3$  & $\lambda_4$  \\ \hline
$ZH\ , \ \nu_e\bar\nu_e H$  &   one-loop  &  two-loop \\
$ZHH\ ,\ \nu_e\bar\nu_e HH$  &   tree  &  one-loop \\
$ZHHH\ ,\  \nu_e\bar\nu_e HHH$  &   tree  &   tree  \\
\end{tabular}
\eeq{eeHHprocesses}
In Ref.~\cite{Maltoni:2018ttu}, both tree and one-loop effects are
included for each process.   Two-loop corrections  are not included.
It is important to note that, while the one-loop effects on single Higgs
cross sections can be computed without reference to an underlying EFT
framework, the one-loop corrections to the $HH$ and $HHH$ cross sections are
UV-sensitive and require renormalisation.  Using the  SMEFT formalism and taking advantage of the 
parametrisation in eq.~\leqn{sixeightL}, the authors of 
Ref.~\cite{Maltoni:2018ttu} worked out these UV-finite expressions.

By changing the values of $c_6$ and $c_8$, one can
independently change the values of $\lambda_3$ and $\lambda_4$.   As
already noted, UV-finite radiative corrections due to $c_6$
and $c_8$  are taken into account.  
The analogous study for 
future hadron colliders, was first  presented in
Ref.~\cite{Borowka:2018pxx}.   This is technically more challenging
because of the need to consider two-loop calculations in the $gg$
fusion channel.   That analysis is described in Sec.~\ref{sec:other_probes}.

With this formalism in hand, Ref.~\cite{Maltoni:2018ttu} presented
constraints on the $ c_6$ and $c_8$ couplings that
would be obtained from the run programs of the proposed $e^+e^-$
colliders
CEPC, FCC-ee, ILC, and CLIC.   The strongest constraints apply to
ILC and CLIC at energies of 500~GeV and above, where \hh and
eventually $HHH$ production is observable.   In this case, we can
consider
the possibility that $c_8$ can be large and quote joint
constraints
on the two variables.   In particular, we can compare the allowed
range of $c_8$ to the theoretical limit 
$c_8\lesssim
31$ quoted in Eq.~\leqn{EFT:c8bound}.  A limitation of this strategy
is that the $HHH$ cross sections at $e^+e^-$ colliders are quite
small. The SM cross sections are shown in Fig.~\ref{fig:HHHcs}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.44\hsize]{HHFuture/fig/xs-vvhhh-nobar.pdf}\ \ 
\includegraphics[width=0.44\hsize]{HHFuture/fig/xs-zhhh-nobar.pdf}\ \ 
\end{center}
\vspace*{-0.4cm}
\caption{Leading order total cross sections for $ZHHH$ (left) and $W$ fusion
  $HHH$ (right)  in $e^+e^-$ collisions, for representative
  values of $c_6$ and $c_8$.  The red solid curves
  are the SM values.  The results refer to
  the ideal beam polarisation choice  $P_{e^-} = -1.0$, $P_{e^+} = +1.0$.}
\label{fig:HHHcs}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-ilc-c6c8.pdf}\ 
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-clic-c6c8.pdf}\\ 
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-ilc-klk4.pdf}\ 
\includegraphics[width=0.47\hsize]{HHFuture/fig/combined-bounds-clic-klk4.pdf}
\end{center}
\vspace*{-0.5cm}
\caption{Combined 90\% CL constraints on the cubic and quadratic Higgs
  self-couplings from the $e^+e^-$ colliders ILC (left) and CLIC
  (right). 
 The upper plots show the 
constraints in the $(c_6, c_8)$ plane; the bottom
plots show the constraints in the $(\kappa_\lambda,\kappa_4)$ plane.
The red regions marked ILC-H and CLIC-H refer to a combination of all
single
 Higgs measurements at all energy stages for each collider under
 study.
 In all cases only the perturbative region described in
 Sec.~\ref{sec:theoretical_constraints_EFT}, $ |c_6| < 5$, $
 |c_8| < 31$,  has been considered. }
\label{fig:Pagani}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In Fig.~\ref{fig:Pagani},  we show as light and dark green regions the
90\% CL regions in this parameter space that would be obtained from
successive stages of running at ILC and CLIC from the measurements of 
$HH$ and $HHH$ production cross sections, assuming that the true
answer is the SM cross section.   The top plots show these 
constraints in the  $(c_6, c_8)$ plane; the bottom
plots show the constraints in the $(\kappa_\lambda,\kappa_4)$ plane.
For ILC, the analysis considers results from $ZHH$ production at
500~GeV  and its combination with results from $ZHHH$ and $W$ fusion
$HH(H)$ at 1~TeV.  (The relevant cross sections for $HHH$ production
are too small to be measured at 500~GeV.) For CLIC, the analysis
considers $ZHH(H)$ and $W$ fusion $HH(H)$ production at 1.4~TeV and 
3~TeV stages.   The luminosities and polarisations assumed are given
in Table~3 of \cite{Maltoni:2018ttu}; these differ in some details
from the current proposals in Refs.~\cite{Bambade:2019fyw} and \cite{Robson:2018enq}.
We also show as red bands the limits on $c_6$ from single
Higgs measurements at ILC and CLIC, using the indirect method
described in the Sec.~\ref{sec:eeindirect}, and assuming that the
two-loop dependence
on $c_8$  is negligible.   The 
CLIC constraints are stronger than ILC ones, thanks to the higher
energies and the greater accessibility of $HHH$ processes. On the
other hand, the $c_6$ constraints from single Higgs
production are stronger 
at the ILC.   Both this constraint and the measurement of $W$ fusion
at higher energies can be used to remove the two-fold ambiguity seen
in the plots for ILC500. Scenarios in which  the measured cross
sections differ from those of the SM have been investigated, assuming
that  they correspond to the more general case $|c_6| < 5$
and and $c_8 = 0$. For positive and large values of $c_6$, the 
constraints on both $c_6$ and $c_8$ 
become stronger than in the SM case, analogously to what we have already 
pointed out in the discussion of Fig.~\ref{fig:HHHBSMresult} for the 
case of $c_6$ only.

The conclusion of this study is that the first coarse bounds on the
value of 
$c_8$,   and in turn on $\lambda_4$, can be set at future
$e^+e^-$
 colliders. The SM rate for triple Higgs
production is not measurable at these $e^+e^-$ colliders, even at the
highest energies considered.  But the cross section strongly depends
on $\lambda_4$, and so it is possible to obtain significant constraints.  
The combination of results from double and triple Higgs production
at high energies improves the constraints.  The $W$ fusion channel
will give  the strongest bounds. For this reason, by increasing the
energy, the precision of the constraints on $\lambda_3$ and
$\lambda_4$ will improve, regardless of the true value of
$\lambda_3$.   
The constraints that can obtained at CLIC at 3~TeV via $W$ boson
fusion $HHH$ production are similar to those that would be obtained
 at a future 100~TeV hadron collider.



 \section{Conclusions}
 \label{sec:eeconclude}

The conclusion of this section have now become clear:
\begin{itemize}
    \item An $e^+e^-$ collider with significant integrated luminosity at
      two different CM energies (e.g., 250 and 350~GeV or 250 and
      500~GeV)  will be able to  determined the Higgs self-coupling
      from measurements of single-Higgs reactions. This determination
      would be robust and 
      model-independent, in the sense that it would be  insensitive to
      the presence of other new physics effects as parametrised by the
      SMEFT.    For currently proposed $e^+e^-$ colliders, the precision on the
      Higgs self-coupling would be 40--60\%, comparable to the
      precision expected from HL-LHC. 
  \item The ILC at 500~GeV would also be able to determine the Higgs
self-coupling from  the measurement of the $ZHH$ production cross
section. 
    This measurement would also  be  robust and 
      model-independent, in the same sense as above.   The expected
      precision on the self-coupling is 27\%. This could be
      combined with the single-Higgs determination to reach a
      precision of  24\%.
    \item The ILC at 1~TeV or CLIC in its proposed program at 1.5 and
      3~TeV would be expected to determine the Higgs self-coupling to
     a precision of  10\% by 
      the measurement of $HH$  production  using the $ZHH$ and
      $\nu\bar\nu HH$ channels.   Though it is likely that this
      measurement would be model-independent in the sense above, that
      issue needs further
      study.
    \item Both the ILC and CLIC programs would provide very strong
      evidence for an increase of the Higgs self-coupling by a factor
      of 2, as actually expected in models of electroweak
      baryogenesis.
    \end{itemize}

    There are reasons to guess that our knowledge of the Higgs
    self-coupling might be even better than that described here.
    First, all estimates from $e^+e^-$ colliders are based on current
    full-simulation analyses.   We have shown  in
    Fig.~\ref{fig:HHHSensitivity} 
     large gaps
    between the results of these analyses and those of ideal analyses with
    perfect signal/background discrimination.   There is considerable
    room to be more clever when we are directly working with data.
    
    Second, these results from $e^+e^-$ colliders will be combined with
    results from $pp$ colliders operating in the same time frame.
     Hadron colliders can be very sensitive to $HH$ production, but there
     are clear difficulties seen today  in extracting model-independent
     estimates of the Higgs self-coupling.  This could be greatly
     assisted by the use of results from $e^+e^-$.   In particular, all
     four proposed Higgs factories are expected to constrain the
     parameter $c_{\Phi G}$ in Eq.~\leqn{lsmeft}, which contributes
     at the tree level in a SMEFT analysis of $gg\to HH$, by measuring
     the $Hgg$ coupling to 1\% precision~\cite{Bambade:2019fyw}.
     Feedback  between $e^+e^-$ and $pp$ measurements will eventually
      lead us to the most precise understanding of the Higgs self-coupling.
 

==> introduction/introduction.tex <==
%\part*{Introduction}

With the discovery of the Higgs boson~\cite{Higgs:1964ia,Higgs:1964pj,Higgs:1966ev,
Englert:1964et,Guralnik:1964eu,Kibble:1967sv} at the Large Hadron Collider~\cite{Aad:2012tfa,
Chatrchyan:2012xdj}, all particles predicted by the Standard Model (SM) of particle physics have now been observed.   However, there remain many questions about the validity of the SM as a fundamental description of nature.  The SM is built around the electroweak gauge symmetry $SU(2) \times U(1)$, which constrains all of the interactions of the model.   
%
Through the precision measurements of electroweak observables,
%Through the precision electroweak experiments of the 1990’s,
we now know that these constraints are obeyed in nature to high precision.   But the electroweak symmetry, if it were exact, would also forbid the generation of mass for all quarks, leptons, and vector bosons.   Thus, this symmetry must be spontaneously broken.   Using our new knowledge of the Higgs boson, we are now in a position to test the predictions of the SM that concern this spontaneous symmetry breaking and its consequences.

From our precise knowledge of the $SU(2)\times U(1)$ coupling constants, the Fermi constant $G_F$ which measures the Higgs field vacuum expectation value $v \simeq 246$~GeV, and the Higgs boson mass $\mh = 125.09\pm0.24$~GeV~\cite{Khachatryan:2016vau}, it is possible to work out the precise predictions of the SM for all other properties of the Higgs boson.  Many of these have been confirmed by LHC measurements of Higgs boson production and decay rates.  For example, the Higgs boson couplings to gluons, to $W$ and $Z$ bosons, and to the fermions of the third generation, are now known to be in agreement with the predictions of the SM to an accuracy of 10--20\%.  


Crucially, though, the Higgs field potential energy function, whose minimum gives the nonzero expectation value that signals spontaneous symmetry breaking, is almost completely unconstrained.  In particular, spontaneous symmetry breaking requires a significant nonlinear self-interaction of the Higgs field, with the potential taking the form
\begin{equation}
V = \frac{1}{2} \mh^2 H^2 + \lHcube v H^3 + \frac{1}{4} \lHquar H^4\,,
\end{equation}
where $\lHcube$ ($\lHquar$) denotes the trilinear (quartic) Higgs self-coupling, and takes the SM value
\begin{equation}
\lHcube = \lHquar = \frac{\mh^{2}}{2v^2}\,.
\end{equation}
These couplings are very weakly constrained by current measurements.   What makes this state of affairs especially troubling is that the SM does not explain why the electroweak symmetry is spontaneously broken.  It only predicts a simple structure of the Higgs potential energy, consistent with the renormalizability of the model.  Alternative models of the Higgs potential, which contain explanations of its form and symmetry-breaking nature, give predictions that are different, sometimes radically so.   Experiment should decide among these models, but, to do that, we need measurements that are sensitive to the Higgs field self-couplings.   


%Though the SM prediction for the Higgs potential seems unremarkable at the energy scale of the weak interactions, the extrapolation of this prediction to very high energy has dramatic consequences for cosmology and for the future of the universe.    Using the current central values of the measurements of the Higgs boson and the top quark mass, this extrapolation produces a potential energy function with a new minimum at Higgs field values above $10^{11}$ GeV.   This implies that the vacuum state of the SM, as we see it today, is unstable, and that, 
%$10^{600}$~years in the future, our universe will be swallowed up in the transition to a new vacuum state with different laws of physics.%~\cite{Buttazzo:2013uya}.  
%It is also possible, within the current uncertainty in the mass of the top quark, that the Higgs self-coupling could tend to 0 at the Planck scale, setting the stage for the Higgs boson to be the inflaton field responsible for the large-scale cosmic structure.%~\cite{Bezrukov:2007ep}.   
%These disturbing or enticing possibilities could be tested with a sufficiently accurate measurement of the Higgs self-coupling.




The measurement of the Higgs self-interaction represents a considerable experimental challenge.
%
The first processes that provide a direct probe to
these couplings are the production of two and three Higgs bosons, since they
involve for the first time the trilinear and quartic Higgs self-couplings at leading order, respectively.
%
The corresponding production cross sections are very small, with the double (triple)
Higgs production rate being about 3 (6) orders of magnitude smaller than for the production of a single Higgs. The experimental sensitivity is further reduced by the presence of large, in some cases irreducible, backgrounds.
As a consequence, the measurement of the quartic coupling is out of reach for the foreseeable future,
while a determination of the Higgs triple self-coupling will require the full integrated luminosity
of the HL-LHC.
%
In addition to the production of Higgs boson pairs, additional information can be
obtained from the indirect effects induced by the
Higgs self-interactions in radiative corrections to electroweak
observables and single-Higgs processes.



Besides being of great importance within the context of the SM,
double Higgs production also provides interesting opportunities for finding new physics beyond the SM. The decay of new resonances into two (not-necessarily-SM) Higgs bosons
can be significant enhanced in a large class of models, turning Higgs pair production into a relevant final state 
for discovering or ruling them out. In addition, the presence of new heavy states in the loop can also alter the non-resonant production rate of Higgs boson pairs, resulting in an enhancement
that could be measured at the LHC. Measuring such an enhancement would strong evidence of new physics, even for scales above the LHC reach.





%The purpose of this report is to summarize the current status of and future prospects for the measurement of the Higgs field nonlinear couplings, and in general for Higgs pair production in the context of the SM and beyond.   
%
%%This report aims to summarize the current status of and future prospects for the measurement of the Higgs boson self-interactions and, in general, of multiple-Higgs production, together with the latest theoretical developments needed for this purpose.
%
This report is subdivided into three parts.
In the first Part of this document we perform a review of the theory of di-Higgs and multiple-Higgs boson production, and the predictions for the Higgs self-coupling in the SM and a variety of alternative models of the Higgs sector.   We then review the current constraints on the Higgs self-coupling from experiments at the LHC—both direct constraints on di-Higgs production and indirect constraints from the systematic uncertainties of Higgs boson couplings to other Standard Model particles—and the prospects for the improvement of these constraints within the LHC program.  Finally, in the last Part we discuss the prospects for the observation and measurement of the Higgs self-coupling at the High-Luminosity LHC and at further future  $e^+e^-$ and hadron colliders.

%This report was initiated as the proceedings of the Double Higgs Production at Colliders Workshop held at Fermilab on Sept. 4-9, 2018.   However, we felt it important to broaden the scope to a general review of current and future measurements of the Higgs self-coupling.   In this way, we hope to provide a resource to guide the development of this subject over the coming years.  The editors would like to thank all contributors, the ATLAS and CMS collaborations, and the LHC Higgs Cross Section Working Group for supporting the preparation of this report and for providing much useful input and advice.

%\section{The Higgs field in the Standard Model and general relativity}
%\input{introduction/SMGRbasics.tex}
%\section{The effective Higgs boson potential}
%\section{Quantum Gravity and asymptotic safety}
%\section{The Higgs boson as an inflaton field}
%\section{The Higgs potential and vacuum stability}
%\section{Higgs boson self-coupling constraints}
%\subsection{Perturbative unitarity constraints on the Higgs boson self-coupling}
%\subsection{Higgs boson self-coupling constraints from electro-weak precision observables}


==> introduction/introduction_new.tex <==
%\part*{Introduction}
In the last decade two important observations have confirmed the general picture at the basis of our current understanding of fundamental physics: 
\begin{itemize}
\item the discovery of the Higgs boson by the ATLAS and CMS collaborations at LHC\cite{ATLASCMS_disc} has set the Quantum Field Theory of the strong and electroweak interaction  (the Weinberg and Salam model)  as a full renormalisable, spontaneously broken, gauge theory, fully predictive up to the energy scale of the Planck mass ($1.22 \times 10^{28}$ eV$/c^2$) and beyond;
\item the observation of the gravitational waves from the LIGO collaboration\cite{LIGO_grav} has finally confirmed the Einstein  theory of general relativity of Einstein.
\end{itemize}

These two theories together are able to describe almost the totality of known phenomena like:  universe expansion, the galaxies and star formation, the stellar evolution,
the radioactivity of nuclei, the particle creation at colliders and their decay properties, and all electromagnetic phenomena.
Phenomena like neutrino oscillations and neutrino masses, that are outside of the Weinberg-Salam model, can be easily described by the addition of 
right handed  neutrinos to the left handed neutrino components in the theory.
More uncertain is the origin of the cosmological expansion, and if these two theories together could provide the elements, like the inflaton field, needed to describe the cosmological evolution of our universe. Moreover, one of the most important missing piece of this model, the so called Cold Dark Matter, needed to properly describe the
cluster galaxy formation, the motion of the stars inside the galaxies and the mulitpole spectrum of the Cosmic Microwave Background, doesn't have a fundamental particle representative in the known Standard Model, but extensive objects, like primordial black holes, could explain the dark matter inside the framework of the standard model and standard gravity.

\section*{The classical formalism}
In the classical formalism (without including quantisation) the two theories can be represented by the classical Hilbert-Einstein action
\begin{equation} \label{eq:action}
S = \int \left [\frac{1}{2}M^2_{\rm pl} R +  \mathcal{L} \right ] \sqrt{-g}d^4x
\end{equation}
where $d^4x$ represents the integral on the space-time coordinates, $g$ is the determinant of the metric tensor matrix $g^{\mu \nu}$, $R$ is the scalar curvature  that
is a function of the second derivatives of $g^{\mu \nu}$, $M_{\rm pl} = \sqrt{\frac{\hbar c}{G}}= 1.22 \times 10^{19}$ GeV/$c^2$ is the Planck mass, $\hbar \sim \frac{h}{2\pi} = 6.582\times 10^{-6}$ eV$\cdot$s is the reduced Planck constant and $G \sim 2.939\times 10^{-62}$ s$\cdot$GeV$^{-1} c^5$ is the Newton gravitational constant.

The SM lagrangian $\mathcal{L}$ is built around the electroweak gauge symmetry $SU(3)_C \times SU(2)_L \times U(1)$, which constrains all of the interactions of the model. It contains three generations of Standard Model fermions, twelve vectorial gauge fields and one scalar  field through the relation:
\begin{align}
\mathcal{L} &= -\frac{1}{4g'^4}B_{\mu \nu}B^{\mu \nu} - \frac{1}{4g^2} tr \left(W_{\mu \nu}W^{\mu \nu} \right) -\frac{1}{4g_s^2} tr \left(G_{\mu \nu} G^{\mu \nu} \right ) \\
&+ \sum_{f=1}^3 i\overline{Q_{Lf}} \slashed{D}Q_{Lf} + i\overline{u_{Rf}}\slashed{D}u_{Rf} + i\overline{d_{Rf}}\slashed{D}d_{Rf} + i\overline{L_f}\slashed{D}L_f  \\ 
&+ i\ell_{Rf}\slashed{D}\ell_{Rf} + \bar{\nu_{Rf}}\slashed{D}\nu_{Rf}  +  \sum_{fk=1}^{3}Y_{u}^{fk}\overline{Q_{Lf}}\tilde{H}u_{Rk} + Y_d^{fk}\overline{Q_{Lf}}Hd_{Rk} \\
&+  Y^{fk}_{l}\overline{L_{Lf}}H\ell_{Rk} +  Y^{fk}_{\nu}\overline{L_{Lf}}\tilde{H}\nu_{k}  -\lambda(H^{\dagger}H)^2 + \lambda v^2H^{\dagger}H-\left(D^{\mu}H \right)^{\dagger}D_{\mu}H \label{eq:potential}
\end{align} 
where the index $f$ runs on the three fermion families, $L$ and $R$ the left and right chirality projections,  $u$ and $d$ indicates the isospin $+1/2$ and $-1/2$ quarks,
$\nu$ and $\ell$ the neutrino and the charged leptons,  $Q_L$ indicates the $SU)2)_L$ quark doublets $(u_L,u_d)$, 
$L_{L}$ the $SU(2)_L$ lepton doublet $\nu, \ell$, $B_{\mu \nu}$ the tensor related to the hypercharge gauge filed, $W_{\mu \nu}$ and $G_{\mu \nu}$ are defined as:
\[
W_{\mu \nu} = \sum_{i=1}^{3} \frac{\tau_i}{2}W^{i}_{\mu \nu} \quad G_{\mu \nu} = \sum_{i=1}^8 \frac{\lambda_i}{2}G^i_{\mu \mu}
\]
where $\tau_i$ are the $SU(2)$ generators represented by the Pauli matrices, and $\lambda_i$ are the $SU(3)$ generators represented by the Gell-Man matrices.
The $tr()$ symbol is intended as the trace over the $SU(2)$ and $SU(3)$ indices, while $W^i_{\mu \nu}$ are the weak $W$ fields  in the weak isospin basis and $G^{i}_{\mu \nu}$ are 
the gluon fields. 

Usually the equation \ref{eq:action} is handled with two different approximation.
A flat space approximation, where the $g^{\mu \mu}$ is constant and, by symmetry principle of general relativity, a global reference frame can be found such that $g^{\mu \nu}$ is equal to the Minkowski metric $\eta^{\mu \nu}$, a diagonal $4\times 4$ matrix with diagonal elements equal to (1, -1, -1, -1). In this approximation, the scalar curvature $R = 0$, and gravity is practically switched off, and all gravitational effects are neglected in the theory.

The action \ref{eq:action} therefore reduces to:
\begin{equation}
\label{eq:action_SM}
    S = \int \mathcal{L}d^4x
\end{equation}
The action \ref{eq:action_SM} can be quantised by the usual canonical quantisation mechanism, and this procedure leads to all predictions of the SM of particle physics.
The vacuum state of the quantised system is defined by the set of values that all fields acquires. In the SM all fields, except the Higgs boson, acquire a null vacuum expectation value. The canonical quantisation is then built around this configuration.  The equation of motion of the vacuum expectation values can be obtained by requiring that a modified version of \ref{eq:action_SM} is stationary, this is know as effective action. Starting from the classical action \ref{eq:action_SM}, standard quantum mechanic methods can be used to compute the effective action and then the equation of motion of the VEVs.

Another way to use action \ref{eq:action} to describe a dynamical system is to ignore completely quantisation and look at a full classical relativistic field theory, where the matter field are described by the lagrangian $\mathcal{L}$. To our knowledge this problem has been attempted with a simplified form of $\mathcal{L}$, including only the neutral electromagnetic field $A^{\mu}$, arising from the mixing of the $B^{\mu}$ and $W_3^{\mu}$ fields, or with the inclusion only of the scalar field $h$, representing the Higgs boson after electroweak symmetry breaking.

In fact, after symmetry breaking the Higgs doublet field $H$ is expressed as: $H = 1/\sqrt{2} (0, v + h)$, where $v$ is the Higgs-boson vacuum expectation value and $h$ is the Higgs-boson field. The potential term in \ref{eq:potential} has the form:
\begin{equation}
V = \frac{1}{2} \mh^2 h^2 + \lHcube v h^3 + \frac{1}{4} \lHquar h^4\,,
\end{equation}
where $\lHcube$ ($\lHquar$) denotes the trilinear (quartic) Higgs self-coupling, and takes the SM value
\begin{equation}
\lHcube = \lHquar = \frac{\mh^{2}}{2v^2}\,.
\end{equation}
From our precise knowledge of the $SU(2)\times U(1)$ coupling constants, the Fermi constant $G_F = 1.1663786 \pm 0.0000006$ measures the Higgs field vacuum expectation value $v = \left (\sqrt{2}G_F \right)^{-1/2} \simeq 246.2196 \pm 0.0002$~MeV, and the Higgs boson mass $125.09\pm0.24$~GeV~\cite{Khachatryan:2016vau}, from which $\lHcube = \lHquar = 0.1291 \pm 0.0005$.
%it is possible to work out the precise predictions of the SM for all other properties of the Higgs boson. 

The last approach is particularly interesting, because it allows to describe  the cosmological inflation as a consequence of the running of the scalar field $\phi$ through the minimum of its potential. The shape of the Higgs potential is therefore a fundamental quantity not only to complete our knowledge of the Standard Model of particle physics, but also to investigate hypotheses on the universe evolution.



    

Through the precision measurements of electroweak observables,
%Through the precision electroweak experiments of the 1990’s,
we now know that these constraints are obeyed in nature to high precision.   But the electroweak symmetry, if it were exact, would also forbid the generation of mass for all quarks, leptons, and vector bosons.   Thus, this symmetry must be spontaneously broken.   Using our new knowledge of the Higgs boson, we are now in a position to test the predictions of the SM that concern this spontaneous symmetry breaking and its consequences.

From our precise knowledge of the $SU(2)\times U(1)$ coupling constants, the Fermi constant $G_F$ which measures the Higgs field vacuum expectation value $v \simeq 246$~GeV, and the Higgs boson mass $\mh = 125.09\pm0.24$~GeV~\cite{Khachatryan:2016vau}, it is possible to work out the precise predictions of the SM for all other properties of the Higgs boson.  Many of these have been confirmed by LHC measurements of Higgs boson production and decay rates.  For example, the Higgs boson couplings to gluons, to $W$ and $Z$ bosons, and to the fermions of the third generation, are now known to be in agreement with the predictions of the SM to an accuracy of 10--20\%.  


Crucially, though, the Higgs field potential energy function, whose minimum gives the nonzero expectation value that signals spontaneous symmetry breaking, is almost completely unconstrained.  In particular, spontaneous symmetry breaking requires a significant nonlinear self-interaction of the Higgs field, with the potential taking the form
\begin{equation}
V = \frac{1}{2} \mh^2 H^2 + \lHcube v H^3 + \frac{1}{4} \lHquar H^4\,,
\end{equation}
where $\lHcube$ ($\lHquar$) denotes the trilinear (quartic) Higgs self-coupling, and takes the SM value
\begin{equation}
\lHcube = \lHquar = \frac{\mh^{2}}{2v^2}\,.
\end{equation}
These couplings are very weakly constrained by current measurements.   What makes this state of affairs especially troubling is that the SM does not explain why the electroweak symmetry is spontaneously broken.  It only predicts a simple structure of the Higgs potential energy, consistent with the renormalizability of the model.  Alternative models of the Higgs potential, which contain explanations of its form and symmetry-breaking nature, give predictions that are different, sometimes radically so.   Experiment should decide among these models, but, to do that, we need measurements that are sensitive to the Higgs field self-couplings.   


%Though the SM prediction for the Higgs potential seems unremarkable at the energy scale of the weak interactions, the extrapolation of this prediction to very high energy has dramatic consequences for cosmology and for the future of the universe.    Using the current central values of the measurements of the Higgs boson and the top quark mass, this extrapolation produces a potential energy function with a new minimum at Higgs field values above $10^{11}$ GeV.   This implies that the vacuum state of the SM, as we see it today, is unstable, and that, 
%$10^{600}$~years in the future, our universe will be swallowed up in the transition to a new vacuum state with different laws of physics.%~\cite{Buttazzo:2013uya}.  
%It is also possible, within the current uncertainty in the mass of the top quark, that the Higgs self-coupling could tend to 0 at the Planck scale, setting the stage for the Higgs boson to be the inflaton field responsible for the large-scale cosmic structure.%~\cite{Bezrukov:2007ep}.   
%These disturbing or enticing possibilities could be tested with a sufficiently accurate measurement of the Higgs self-coupling.




The measurement of the Higgs self-interaction represents a considerable experimental challenge.
%
The first processes that provide a direct probe to
these couplings are the production of two and three Higgs bosons, since they
involve for the first time the trilinear and quartic Higgs self-couplings at leading order, respectively.
%
The corresponding production cross sections are very small, with the double (triple)
Higgs production rate being about 3 (6) orders of magnitude smaller than for the production of a single Higgs. The experimental sensitivity is further reduced by the presence of large, in some cases irreducible, backgrounds.
As a consequence, the measurement of the quartic coupling is out of reach for the foreseeable future,
while a determination of the Higgs triple self-coupling will require the full integrated luminosity
of the HL-LHC.
%
In addition to the production of Higgs boson pairs, additional information can be
obtained from the indirect effects induced by the
Higgs self-interactions in radiative corrections to electroweak
observables and single-Higgs processes.



Besides being of great importance within the context of the SM,
double Higgs production also provides interesting opportunities for finding new physics beyond the SM. The decay of new resonances into two (not-necessarily-SM) Higgs bosons
can be significant enhanced in a large class of models, turning Higgs pair production into a relevant final state 
for discovering or ruling them out. In addition, the presence of new heavy states in the loop can also alter the non-resonant production rate of Higgs boson pairs, resulting in an enhancement
that could be measured at the LHC. Measuring such an enhancement would strong evidence of new physics, even for scales above the LHC reach.





%The purpose of this report is to summarize the current status of and future prospects for the measurement of the Higgs field nonlinear couplings, and in general for Higgs pair production in the context of the SM and beyond.   
%
%%This report aims to summarize the current status of and future prospects for the measurement of the Higgs boson self-interactions and, in general, of multiple-Higgs production, together with the latest theoretical developments needed for this purpose.
%
This report is subdivided into three parts.
In the first Part of this document we perform a review of the theory of di-Higgs and multiple-Higgs boson production, and the predictions for the Higgs self-coupling in the SM and a variety of alternative models of the Higgs sector.   We then review the current constraints on the Higgs self-coupling from experiments at the LHC—both direct constraints on di-Higgs production and indirect constraints from the systematic uncertainties of Higgs boson couplings to other Standard Model particles—and the prospects for the improvement of these constraints within the LHC program.  Finally, in the last Part we discuss the prospects for the observation and measurement of the Higgs self-coupling at the High-Luminosity LHC and at further future  $e^+e^-$ and hadron colliders.

%This report was initiated as the proceedings of the Double Higgs Production at Colliders Workshop held at Fermilab on Sept. 4-9, 2018.   However, we felt it important to broaden the scope to a general review of current and future measurements of the Higgs self-coupling.   In this way, we hope to provide a resource to guide the development of this subject over the coming years.  The editors would like to thank all contributors, the ATLAS and CMS collaborations, and the LHC Higgs Cross Section Working Group for supporting the preparation of this report and for providing much useful input and advice.

%\section{The Higgs field in the Standard Model and general relativity}
%\input{introduction/SMGRbasics.tex}
%\section{The effective Higgs boson potential}
%\section{Quantum Gravity and asymptotic safety}
%\section{The Higgs boson as an inflaton field}
%\section{The Higgs potential and vacuum stability}
%\section{Higgs boson self-coupling constraints}
%\subsection{Perturbative unitarity constraints on the Higgs boson self-coupling}
%\subsection{Higgs boson self-coupling constraints from electro-weak precision observables}


==> introduction/preface.tex <==
\indent With the discovery of the Higgs boson~\cite{Higgs:1964ia,Higgs:1964pj,Higgs:1966ev,
Englert:1964et,Guralnik:1964eu,Kibble:1967sv} at the Large Hadron Collider~\cite{Aad:2012tfa,
Chatrchyan:2012xdj}, all particles predicted by the Standard Model (SM) of particle physics have been observed, however many predictions of the model still need to be tested.
The Large Hadron Collider running between Switzerland and France from the year 2009 to 2018 has, in fact, provided measurements of the Higgs  boson couplings to the vector bosons $W$ and $Z$ and to the heaviest generations of quarks and charged leptons,  while couplings to the first two generations and to neutrinos are still completely untested. Moreover, the energy potential of the Higgs boson field that is responsible for the electroweak symmetry breaking 
is still completely untested.

The Higgs boson potential has a simple polynomial expression in even powers of the Higgs boson field up to the fourth. After the electroweak symmetry breaking, a cubic term in the Higgs field is generated that induces a Higgs boson self-interaction (self-coupling), that is proportional to a dimensionless parameter $(\lambda)$. The $\lambda$ value runs with the energy scale, that results in an effective potential that has a non trivial behaviour for large values of the Higgs boson field. 

The shape of the effective  potential is particularly interesting because it has deep theoretical and cosmological consequences. In fact, within the current uncertainty in the mass of the top quark $\lambda$ could tend to zero at the Planck scale. In this case, it has been advocated \cite{Shaposhnikov:2009pv} that a quantum gravity theory can be built starting from the present formulation of the general relativity and the Standard Model of particle physics,  that is fully renormalisable in a non-perturbative manner.
In addition, in the case of a non-minimal coupling between the Higgs field and the gravity, \cite{Bezrukov:2007ep}, or new physics contribution \cite{Masina:2011aa},
 the Higgs boson field could act as an inflaton field and therefore be responsible of the cosmological inflation. 
%setting the stage for the Higgs boson to be the inflaton field responsible for the large-scale cosmic structure.%~\cite{Bezrukov:2007ep}.  
Finally, using the current central values of the measurements of the Higgs boson and the top quark mass, the Higgs potential energy function has a new minimum at Higgs field values above $10^{11}$ GeV.   This implies that the vacuum state of the SM, as we see it today, is unstable, and that,  $10^{600}$~years in the future \cite{Cabibbo:1979ay,Buttazzo:2013uya,Degrassi:2012ry} , our universe will be swallowed up in the transition to a new vacuum state with different laws of physics.
These disturbing or enticing possibilities could be tested with a sufficiently accurate measurement of the Higgs self-coupling.

The value of the Higgs boson self-coupling is predicted in the SM to be a function of the Higgs boson mass, \mH and the Fermi coupling constant $G_F$, its value is therefore completely determined by these two observables. Nevertheless this prediction is still far to be tested, because all precision observables show a loose dependence on $\lambda$. Constraints on $\lambda$ derive from perturbative unitarity arguments, but also in these cases they are quite weak, spanning up to five times the SM predicted value. Furthermore, unitarity can be restored by non perturbative effect like di-Higgs resonance production, therefore the validity of such constraints are strongly model dependent.

The target of the present work is to summarise the present status of the di-Higgs boson production search and indirect constraints on the value of $\lambda$, with the wish to serve as a useful guide for people working on di-Higgs production or Higgs boson self-coupling in the next years. The work has started as the proceedings of the Di-Higgs workshop at Colliders, that was held at Fermilab from the 4th to the 9th of September 2018, but it went beyond the topics discussed at that workshop and included further developments. The editors would like to thank all contributors, the ATLAS and CMS collaborations and the Higgs cross section working group 
for supporting the editing of this white paper and for providing many useful inputs and advises,  and in particular Michael Peskin for his careful review of the manuscript and his substantial contribution to the overall shaping of this work.
%
\vspace*{2cm} \\
\phantom{x}\hspace{10cm}{\Large The  editors}\\
\phantom{x}\hspace{10cm}{\large \textit{B. Di Micco}}\\
\phantom{x}\hspace{10cm}{\large \textit{M. Gouzevitch}}\\
\phantom{x}\hspace{10cm}{\large \textit{J. Mazzitelli}}\\
\phantom{x}\hspace{10cm}{\large \textit{C. Vernieri }}



==> ref_requets.tex <==
Dear Colleague,

We are going through your recent paper on Higgs boson pair production at colliders: status and perspectives (https://arxiv.org/abs/1910.00012) with great interest.

We would like to draw your attention to our work https://arxiv.org/abs/1812.05640, on Resonant heavy Higgs searches at the HL-LHC. One of the primary objectives of this work were that we calculated production cross-section limits from multifarious heavy Higgs decay channels in a model-independent way and draw its impact on the MSSM parameter space at the HL-LHC.

We hope that you find our work relevant.
  
Thank you very much.

Best regards,
Amit
(On behalf of the authors)

Dear Javier, et al. --

In re-reading your email just now, I realize that I did not respond to the actual question you asked, namely, where in your review we would suggest your citing our work. I apologize for my careless oversight. In our opinion, the most obvious place for a citation would be within a discussion of two-Higgs-doublet models (2HDM) as presented in the well-known review paper by Branco, et al. Although our scale-invariance-based GW model is distinctly different from the garden-variety 2HDM's covered in Branco, that is still its natural home.

In looking more carefully at your paper, however, especially Chapter 3, I see no dedicated discussion anywhere of the effect on di-Higgs production of the simple 2HDM's Branco, et al. discussed. Frankly, I'm surprised by this given the amount of attention these 2HDM's receive in ATLAS and CMS papers on searches for new charged and neutral Higgses. So, embarrassingly, this leaves me at a loss as to where you might cite our work. I would be grateful for your advice on this.

Thank you again for your kind reply.

  Best regards,

  Kenneth Lane
  Eric Pilon
  
  
  Dear Biagio and Suyog,

I am writing you according to a conference paper that came out recently about Higgs Boson pair production at colliders, where your main contribution was focused on the HH→bbWW* channel (sections 5.4.2 and 5.4.3).

I would like to point out that this specific search was study for the first time by me and other collaborators in the context of BSM extension:

"Resonant Higgs boson pair production in the hh→bbWW*→bbℓ+νℓ−ν decay channel"

http://inspirehep.net/record/1339393

https://arxiv.org/abs/1501.03799

(our paper is for example cited in the same conference paper in the section 3.1, reference [195])

As you can see there, the process studied is the one that now ATLAS is capable to study. There we performed a complete study using the mT2 variable as it is suggested in section 5.4.3. I would appreciate if you could please have a look at the paper since we were the first people approaching this channel properly for a heavy resonant Higgs boson decaying into two SM Higgs bosons, but somehow it has been forgotten by the experimental groups when performing the search and it has not been cited. 
In any case I would be very grateful if you could give me your opinion about the paper and the analysis that we did and also if it could be of any help for the actual ATLAS search. Furthermore, we are open also to help, collaborate or be of any help for this process.

I hope you could find our paper interesting.

Best regards,

Víctor.

https://docs.google.com/document/d/1gWQUSH7wgAlja8ciPHbgzXaRIEB6xSJxtmSpb3KMks8/edit?usp=sharing

